An Empirical Study on the Bugs Found while Reusing Pre-trained Natural Language Processing Models

In NLP, reusing pre-trained models instead of training from scratch has gained popularity; however, NLP models are mostly black boxes, very large, and often require significant resources. To ease, models trained with large corpora are made available, and developers reuse them for different problems. In contrast, developers mostly build their models from scratch for traditional DL-related problems. By doing so, they have control over the choice of algorithms, data processing, model structure, tuning hyperparameters, etc. Whereas in NLP, due to the reuse of the pre-trained models, NLP developers are limited to little to no control over such design decisions. They either apply tuning or transfer learning on pre-trained models to meet their requirements. Also, NLP models and their corresponding datasets are significantly larger than the traditional DL models and require heavy computation. Such reasons often lead to bugs in the system while reusing the pre-trained models. While bugs in traditional DL software have been intensively studied, the nature of extensive reuse and black-box structure motivates us to understand the different types of bugs that occur while reusing NLP models? What are the root causes of those bugs? How do these bugs affect the system? To answer these questions, We studied the bugs reported while reusing the 11 popular NLP models. We mined 9,214 issues from GitHub repositories and identified 984 bugs. We created a taxonomy with bug types, root causes, and impacts. Our observations led to several findings, including limited access to model internals resulting in a lack of robustness, lack of input validation leading to the propagation of algorithmic and data bias, and high-resource consumption causing more crashes, etc. Our observations suggest several bug patterns, which would greatly facilitate further efforts in reducing bugs in pre-trained models and code reuse.

==> challenges.tex <==
\section{Discussion}
\label{sec:challenges}
\paragraph{Black Box Analysis.}
\label{subsec:blackbox}
Although dataset are generally available to the developers, most ML models are black-box in terms of the learning process and model structures. Language models are not an exception. Even though the model functionalities are accessible, the implementation details are hidden inside the model structure. If we think of the language model as a monolithic block, then certainly abstraction has been created to provide controllable parameters to the developers and make changes at a small scale. This is similar to extending a class and change the public section of the parent class. It hides the details of the underlying algorithms from the users. For instance, a developer wants to build a language model for Khmer' language~\cite{blackbox2}. Due to the unavailability of the underlying architecture or the actual dataset used to train \bert, the developer
is finding it difficult to alter the task.
%\begin{figure}[!htp]
%	\includegraphics[scale = .4, width=\linewidth]{blackbox2.png}
%	\caption{Developer Facing Difficulty in Understanding Underlying Impletation.~\cite{blackbox2}}
%	\label{fig:blackbox}
%\end{figure}
Here, from a developer's perspective, an in-depth analysis of each of the layers and the dataset will help to come up with a better understanding of the changes that need to be done. 


%In general, abstraction means creating an interface around a code
%that will hide the implementation level details and give the developers only
%what they need for task-specific implementation. If we think of the language
%model as a whole single, monolithic block, then certainly abstraction has been
%created to provide controllable parameters to the developers and make changes
%at a small scale. This is similar to extending a class and change the public
%section of the parent class. It insulates users from the detailing of the
%underlying algorithm. 
%
%Each language model is capable of performing specific downstream tasks. The
%reason to create this abstraction is that such vast language models are not
%readily understandable. For such scenarios, these models are like clean
%interfaces with specific system functionalities available for the developers
%even though the interface is accessible by the users; however, the
%implementation details are hidden inside the black box. 
%
%Since the state-of-the-art result is achievable using these language models on
%the mentioned dataset along with a set of hyper-parameters. When we use a
%framework for implementing a certain task, at the core level, we are creating a
%mapping from such tasks to a lower level of functionality. So, an in-depth
%analysis of the functionalities of each of these modules or interfaces will
%help the developers to further granulate their understandings of the methods
%and modify them as per their requirements. However, because of the complex
%architecture of these language models, analysis becomes a cumbersome task. 
%
%So the question is, when such conflicts arise? Conflict arises when a developer
%wants to change certain attributes of the pre-defined language models as per
%their need like in Figure \ref{fig:blackbox} shows that how a developer is
%facing issue for all such words that can be written using abbreviation like
%'Could replace with Cud' While performing sentiment analysis as a downstream
%task, the critical words driving the sentiment should be 'better'; however,
%maximum attention score has been given to '\#\#i,' which has no significant
%contribution to sentiment analysis. Here, from a developer's perspective, an
%in-depth analysis of each of the layers along with the shared interfaces will
%help them to come up with a better distribution of scores. 

%\paragraph{Scalability and the Impact on Environment.}
%%If a model is trained at a small scale, however, if the same is used for
%%large-scale implementation, then it outputs considerable accuracy with minimal
%%compromise. Even though trained on a small corpus in a specific environment,
%%the same model will make the best utilization to learn when implemented for
%%large corpus and diverse backgrounds. Then we will say that the model is
%%scalable.
%
%Language models are trained on an enormous corpus, and each of them is specialized for performing certain tasks. For instance, Google has a multilingual model (\textit{mBERT}), trained on a corpus of 104 languages. In the past few years, we have seen an impressive performance from BERT models trained on a specific language however extension of the model to support multi-languages is an example of scalability. However, ~\citeauthor{wu2020all}~\cite{wu2020all} showed that \textit{mBERT} performs better for languages that have large resource availability but perform poorly for small resource languages. Similarly, \roberta, a language model, is developed using improved version of hyper-parameters and increased dataset in comparison to \bert. However, when we consider scaling a model, then it should not be considered only in terms of increasing the architectural size to upgrade the performance. Prior works~\cite{jiao2020tinybert, sanh2019distilbert} have shown that down-scaling the language model has given effective and considerable performance on multiple tasks and natural language dataset.



%However, X~\etal discussed that
%\bert models are not scalable in the sense that not many parameters or the white-box section in the whole learning pipeline. Due to this such restrictions often, a new model is needed to perform a little better with changing the structure of the problem. For example, the \roberta is a model that builds on top of the \bert with X, Y, Z addition.
%Mohna: add X, Y , and Z

%Scalability of the language models has a direct relationship with environmental impacts making it important for the developers to re-examine and re-validate the design process. Recently, it has been noticed that the cost of training model has a direct impact on the environment.  Instead of rebuilding the models to add more data or changing the structure of the model, more scalability should be added so that the current version of the models can be applied for more tasks rather than creating a new one.


\paragraph{Library support and incompatibility}
\label{subsec:scalability}

Most of the pre-trained models have been implemented from emerging research results. A few of them are available through popular deep learning libraries such as \tensor and \torch. However, the core model implementations are still in active development. API structure for the models are often pre-configured with
specific requirements, which resulted in many API and structural bugs. Developers often fail to capture the tight specification from usage examples and documentation. In addition, NLP tasks also need a number of data and platform-specific steps, which are not supported by the pre-trained models locally. For example, to build a sentiment classifier on new dataset using \bert, developers would need to prepare data using external libraries such as \textit{pandas}, \textit{NumPy}, etc., and set up GPU training backend using \tensor, and so on. Therefore, several
dependencies among libraries occur, which are implicit in many cases, causing fatal bugs for the developers. Therefore, there is an immediate need to address the specification and dependency issues by the library developers and researchers. 




==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\begin{enumerate}
   %% this sentence doesn't make sentece >> 
    \item Since NLP tasks require models trained on very large corpus, reusability, replicability and modular software engineering are immediately required. 
    %% <<
\red{
   \item NLP pre-trained models usage is still in its infancy. The models we studied are under active development. Continuous improvement and maintenance of the models require a unified framework and methodologies. 
  \item Our study shows many opportunities to identify the bugs automatically by static analysis. 
  \item Many of the bugs can be fixed by automated repairs. We need more repair tools that leverage both static and dynamic analysis. Furthermore, the interaction between data and model should be made more explainable. 
  \item Finally, the black-box nature of pre-trained models is the reason for many bugs in the client code. The usability of the APIs is also bug concern. More research is needed to enhance the software architecture and design of the NLP models.
  }
\end{enumerate}

==> nlp (Version 920)/NLParam.tex <==
%\subsection{Confusion in NL-specific Specifications}
\subsection{What are the most bug prone NL-specific parameters?}
\begin{figure}[!htp]
	\centering
	\includegraphics[width=0.8\columnwidth]{cnls}
	\caption{Example of the wrong specification~\cite{cnls}}
	\label{fig:cnls}
\end{figure}
A majority of the bugs (21.4\%) are caused by using a wrong parameter
while reusing the NL models. Most such cases are caused due to the black-box nature of these models. Developers choose to tune these parameters without knowing the internals of the model. Moreover, such practices often go beyond the accuracy of the model and impact on robustness, fairness, and other properties of the model. Here, we discuss these NL-specific parameters and other specifications, e.g., tokenization, language, vocabulary; developers can alter that. Also, we describe how different choices would impact the model's behavior. For instance, Figure~\ref{fig:cnls} shows an example where the developer is having trouble reusing the \bert model to perform a certain task in the Devanagari language. There is a concept of compound letters in this particular language, where two vowels can be combined to form another letter (as suggested by the developer in the issue). Since such knowledge is not present in the reused model, the tokenizer only works on the first vowel of the compound letter. Such bugs are related to the wrong specification of the upstream and the downstream software. Here, we discuss such types of root causes in detail. %Moreover, we found that bugs due to IPS or incorrect model parameter or structure in traditional DL are similar to 

\finding{Wrong NL batch size and sequence length can affect the robustness of the NL software.}

\subsubsection{Batch Size}
Among all the NL-related parameter settings, setting up the correct \textit{Batch Size} is the cause for most of
the bugs (21.76\% of bugs in this category (4.65\% overall)). Batch size controls the flow of the input to the model while training. Every model is shipped with a default value for this parameter. However, to accommodate the model and execute on the tailored problems, one might need to alter the value of this parameter. The value can either be increased or decreased based on the need and the available resources. However, both options have their pros and cons.
%For instance, lowering the batch size can help to accommodate a large model.
% as shown in Figure \ref{fig:batch}.
%\begin{figure}
%	\includegraphics[width=\linewidth]{batch}
%	\caption{Memory Out of Bound due to wrong Batch size~\cite{batch}}
%	\label{fig:batch}
%\end{figure}

\textbf{Decreasing the Batch Size.} 
36.96\% of the bugs caused by the batch size end up having memory
issues, and the other 34.78\% halts the program abruptly. We found that all the bugs
related to the memory issue have a common fix: decreasing the batch size to
accommodate the program with limited resources. However, developers are unaware that, while decreasing the batch size will reduce the memory consumption
and make the learning process faster, it might also decrease the robustness. If the NLP
model is related to a safety-critical system or dataset with sensitive
information, then decreasing the batch size will jeopardize the system's safety. NLP, as well as
most DL architectures, use a stochastic gradient-based approach for
learning. With a fixed batch size, the gradient computation approximates the
loss between two input batches. If a developer decreases the batch size
significantly, then computed approximation will have high variance, and it will
direct the model to learn faster. Small batch size often helps skip some local minima
and contribute to the right direction~\cite{mccandlish2018empirical}. However, if the batch size is
extremely small, then two things can happen. First, if the dataset has a bias
towards a particular word, then sample bias could be created, and the model will
try to remember the word. If an adversary changes the word to a different word,
then it will decrease the overall robustness of the
model~\cite{galloway2019batch}. For instance, there is a sample bias over the
word ``dog'' in a dataset. %and with a small batch size, the context of the
%word depends on the word. 
If a sentence, ``Dog is barking'' is classified as negative and the
adversary only changes the ``barking'' with ``eating'',
then the sentence will be classified as negative as well, which is incorrect. Here, due to the small batch size, the model starts to remember the words associated with the sentiment and predicts if there is a presence of such words without validating other sections of the sentence. Second, if the batch size is very small, the model might never converge and will never halt, and thus, it will not
reach the desired accuracy, which will make the NLP system vulnerable to adversarial attacks.


\textbf{Increasing the Batch Size.} 
While decreasing batch size will
decrease the robustness, increasing the batch size can also have adverse
effects. If the batch size is too big, then the approximation
between the two batches of input is too large, which will not help
the model learn and take more iteration to converge. This is the
primary reason for having memory out of bound error. 

\textbf{\textit{Implications.}} There is no optimum value for the batch size that can help the
model be more robust. Runtime verification could be done on the gradient
approximation to identify such issues. This could be done at either API level,
e.g., TensorFlow and PyTorch APIs, or by building a
dynamically analyzing gradient approximation. If the value
exceeds a certain threshold, developers could either be informed or the program
can be halted.

\subsubsection{Sequence Length.}
\begin{figure}
	\includegraphics[width=1\linewidth]{max}
	\caption{Solution to a max length related bug~\cite{max}}
	\label{fig:max}
\end{figure}
16.20\% (3.46\% overall) NL-specific parameter-related bugs are due to setting incorrect
sequence length, which can affect the robustness of the system.
The model creators commonly set up the sequence or max length. This parameter limits
the length of the sentence that can be processed at a time. For instance, \bert
and \roberta have a maximum allowable sequence length of 512. While this
constraint can certainly help the model perform better, it can have adverse
effects. 
If the average length of the sentences in a dataset is more than the max length,
then the model may not learn the reference, which the adversary can utilize
to break functionalities. For instance, as shown in Figure \ref{fig:max}, the
sentence ``The man went to the store and bought a gallon of milk'' will be split
between two parts, 1) ``the man went to the store'', and 2) ``and bought a
gallon of milk'' based on the restriction imposed by the sequence length (for illustrative purpose, we take sequence length as 6).
Due to the constraint on the parameter, the meaning of the sentence is lost, and
an adversary can change a single word. For
example, if the word ``store'' is changed to ``mars'', the first
part of the sentence can still be valid. But
without the imposed constraint, two sentences will not be split, and the semantic will be preserved. 
In the same figure, the author of the post, a co-author of \bert suggested that a data split can help escape such problems.

\textbf{\textit{Implications.}}
There are works to auto-tune hyper-parameters in the 
DL~\cite{deng2013new, ilievski2017efficient} and SE~\cite{fu2017easy, arcuri2011parameter} domains. For instance,
AutoML~\cite{he2021automl} uses neural architecture search (NAS) for parameter
optimization. A similar architecture could be used for the NL domain. While
optimizing the parameters, besides accuracy, other non-functional properties should also be
taken into account. In SE, works on search-based
systems~\cite{arcuri2013parameter, agrawal2018wrong} have proposed different
techniques to identify the near-optimum value for the hyper-parameters. Such
systems could be used to tune the hyper-parameters in NL-specific software.

\subsubsection{Language.} 
\finding{Improper language specification can propagate bias in NLP pre-trained models.}
\begin{figure}[!htp]
	\includegraphics[width=1\linewidth]{language}
	\caption{Natural language specification bug ~\cite{language}}
	\label{fig:language}
\end{figure}
16.67\% (3.56\% overall) of bugs related to the wrong specification of NL-parameters are due to the wrong use of NL specifications while reusing the models. For instance, Figure~\ref{fig:language} shows an issue that a developer faces while reusing the multilingual \bert for the Chinese language. Since there is no whitespace needed to separate words in Chinese, the multilingual pre-trained model often confuses while tokenizing. The pre-trained model is trained on the English dataset, and the same has been used to create the embedding of the Chinese language. However, the issue occurs due to the mismatch between the specifications of the two natural languages. While these issues can cause wrong translation by introducing whitespace, often it can invoke gender bias, too. For example, the words in English are not gender-specific, whereas
languages like Spanish, French, Hindi, etc., have gender-specific words. For
instance, in Spanish, the word ``doctor'' is either ``doctor'' (male) or
%\begin{figure}
%%	\includegraphics[width=1\linewidth]{bias}
%	\caption{Example of Language Bias~\cite{bias}}
%	\label{fig:bias}
%\end{figure}
``doctore'' (female) based on the actor in the sentence.
If a model is built to translate sentences from English to Spanish, then when
the gender-specific words are encountered, the model will depend on the context
of the surrounding words. For instance, when ``My friend is a doctor''
is translated to Spanish, it can either be considered as, 1) ``Mi amigo es doctore'' (female), or 2) ``Mi amigo es doctor''
(male)~\cite{johnson2020scalable}. However, due to the presence of gender bias in
the English dataset, the system
predicts the second option or the male version. 
% A similar example is shown in Figure~\ref{fig:bias}, where the translation from English to Romanian losses some key aspects. 

\textbf{\textit{Implications.}} Recently, ML models are accused of propagating bias or unfairness in the prediction \cite{galhotra2017fairness, aggarwal2019black, udeshi2018automated}. The NLP models also exhibit such bias because of their nature and reuse scenario. 
Based on the above finding, we think a formal specification should be incorporated while building such models. This is akin to introducing contracts in software development. If we compare the source language as the subtype of the target language, then a specification could be built around the multilingual translation that will validate the operation beforehand. The source language should have all the target language characteristics and more. For instance, if one of the meta-variable on which the contract can be invoked is gender, then the value corresponding to the English language will be gender-neutral, whereas it will be gender-specific for Spanish. Having such specifications can warn the developers about information loss.

\finding{Bugs can occur due to incorrect semantic preservation.}
\subsubsection{Tokenization.} 
%\begin{figure}
%	\includegraphics[width=1\linewidth]{tokenizer}
%	\caption{Example of Tokenization-related Issue.~\cite{tokenizer}}
%	\label{fig:tokenizer}
%\end{figure}
24.07\% (5.15\% overall) of parameter-related bugs occur because of wrong tokenization,
mostly ending up crashing (68.2\%) the system. In NLP-based systems, tokenization has
been done to preserve the semantics of the input dataset and dismantle the input
dataset into smaller units, where the units can be word, sub-word, or a
character. 
% For instance, \bert performs tokenization in two ways. First,
% splitting the input sentence based on space, punctuation, etc. Second, by
% converting the input sentence into meaningful word chunks as per its pre-defined
% vocabulary. For unseen words, the second approach converts a word into the longest sequence of the available words as per its vocabulary. 
% In issue~\cite{tokenizer}, a developer using \bert for tokenizing a custom text that has emoji. Since the pre-trained model does not support emoji, the sentence ``I \heart you" has been tokenized into ['i', [UNK], 'you'], where [UNK] denotes the missing token. Since the context of the sentence was represented using the emoji, wrong tokenization losses the key meaning of the sentence.
\begin{figure}
	\includegraphics[width=1\linewidth]{tokenizer2}
	\caption{Example of tokenization-related bug~\cite{german}}
	\label{fig:tokenizer2}
\end{figure}
% Another example is shown in 
For instance, we show an example in Figure~\ref{fig:tokenizer2}, where a developer builds a model to translate German sentences into
English sentences. A model trained with the English language has been reused. If an unseen word occurs in the German language, wrong token
representation can lose the semantics of the input language. For instance,
``Hallo'' in German means ``Hi''. If the pre-trained model is reused to translate
``Hallo'', then the output of the tokenization step could be ``Hall'',
``\#\#o''. Surprisingly, there is a word ``Hall'' in the English vocabulary. In this scenario, the semantics of the word ``Hallo'' is not preserved.

% \subsubsection{Vocabulary Size.}
% While retraining a model with a dataset, a user needs to provide the vocabulary
% size of the model. Since there is a constraint on the maximum limit of the vocabulary
% size, developers often face trouble deciding how to load their custom dataset. Also,
% due to the size constraint, the semantics of the language could not be preserved.
% For instance, an issue while reusing \roberta~\cite{vocab}, where the developer wants to upload
% a corpus of Brazilian tweets, and the program crashed because the size of the
% vocabulary exceeds the pre-determined size in \roberta. A solution to this bug
% is to truncate the corpus, but that may lead to losing key information.

%\begin{figure}
%	\includegraphics[width=.9\linewidth]{vocab}
%	\caption{Example of Vocabulary Size Mismatch.~\cite{vocab}}
%	\label{fig:vocab}
%\end{figure}

\textbf{\textit{Implications.}}
In SE and PL, vast works~\cite{ouni2012search, chlipala2007certified, zhao2012formalizing} has been done to preserve the
semantics of the code during code translation. Also, a proof checking-based
approach can be implemented to validate the semantics of the source and the
target language. 
Recently, \citeauthor{lagouvardos2020static}~\cite{lagouvardos2020static} have proposed a Tensor type to validate the tensor-based operations in DL.
Such type of system can help in the NLP domain to formally prove the preservation and progress.

The rest of the (20.5\%) bugs in this category are caused due to the incorrect choice of the vocabulary length and wrong sentences given in the dataset.

==> nlp (Version 920)/abstract.tex <==
In Natural Language Processing (NLP), reusing pre-trained models instead of training from scratch has gained a lot of popularity; however, these models are mostly black-boxes, extremely large, and building a model from scratch often requires significant resources. To ease, models trained with large corpora are made available, and developers reuse them in different problems. In contrast, developers mostly build their models from scratch for traditional deep learning (DL)-related problems. By doing so, they have full control over the choice of algorithms, data-processing, model structure, tuning hyperparameters, etc. Whereas in NLP, due to the reuse of the pre-trained models, NLP developers are limited to very little to no control over such design decisions. They can either apply tuning or transfer learning on pre-trained models to meet their requirements. Also, NLP models and their corresponding datasets are significantly larger than the traditional DL models and require heavy computation. Such reasons often lead to bugs in the system while reusing the pre-trained models. While bugs in traditional DL software have been intensively studied, the nature of extensive reuse and black-box structure motivates us to understand the different types of bugs that occur while reusing NLP models? What are the root causes of those bugs? How do these bugs affect the system?
To answer these questions, we studied the bugs reported while reusing the 11 popular NLP models. We mined 9,214 issues from their respective \textit{GitHub} repositories and identified 984 bugs. We created a taxonomy with the bug types, root causes, and impacts. Our observations led to several key findings, including limited access to model internals resulting in lack of robustness, lack of input validation leading to the propagation of the algorithmic and data bias, high-resource consumption causing more crashes, and memory-out-of-bound errors,  etc. Our observations suggest several bug patterns, which would greatly facilitate further research and development for reducing bugs in the pre-trained models as well as the code that reuses them.

==> nlp (Version 920)/bugtype.tex <==
%The bugs in reusing NLP models are broadly classified into four categories.
%: API, Data,
%Structural, and Non-Structural Bug. There are several sub-categories within
%structural bug types that discuss the different bug types related to the model
%structure. For non-structural bug types, we found that only an initialization
%bug is observed while reusing pre-trained models in NLP. %For non-structural bug
%Here, we briefly describe the bug types.

\textbf{API Bug.} 
%This kind of bug occurs due to reusing the APIs of the NLP models provided by different libraries such as \tensor, \torch, etc.
API-related issues are mostly due to the
changes in the top-level APIs that cause the models to behave aberrantly. 
These types of bugs can occur both from misuse by the developer of the client code as well as for missing the compatibility among the
APIs. 
%Often, bugs are caused due to missing compatibility among all the APIs
%involved in the system.
%For example, in the following code snippet \cite{apibugex}, the user is reusing the \bart model from \tensor library. But the \texttt{MBartTokenizer.from_pretrained} API has not been used correctly due to the confusion in the documentation.
%
%\begin{lstlisting}[language=Python]
%example_english_phrase = "UN Chief Says There Is No Military Solution in Syria"
%expected_translation_romanian = "SOME TEXT"
%batch = MBartTokenizer.from_pretrained('facebook/mbart-large-cc25').prepare_seq2seq_batch(example_english_phrase, src_lang="en_XX", tgt_lang="ro_RO", tgt_texts=expected_translation_romanian)
%input_ids = batch["input_ids"]
%target_ids = batch["decoder_input_ids"]
%\end{lstlisting}

\textbf{Data Bug.} When bugs are caused while loading the training data for the NLP models, we refer to them as data bugs. 
%Since reusing the models is mostly about using the models with customizing data and parameters, software that uses these model are more focused on the data than other domains of the machine learning problems. 
%Bugs in data can be triggered by the wrong data type, size of the data, etc.

\textbf{Structural Bug (SB).} This genre of bugs is associated with the
incorrect definition of the model structure. 
Bugs associated with the structure of the model is classified further into five categories:
\begin{enumerate}[leftmargin=*]
	\item \textbf{Control and Sequence Bug:} These bugs are related to the control sequence or control flow of the code.
	\item \textbf{Data Flow Bug:} While data bugs are related to the input data,
	data flow bugs are referred to as the bugs seen when data passes through the
	model structure. For instance, the output shape of the data after applying a layer operation does not match with the input required for the operation of the consecutive layer. In such cases, we classify the bugs as data-flow bugs.
	\item \textbf{Initialization Bug:} Reusing the NLP models involves the initialization of
	different hyper-parameters. These parameters help define the vocabulary size, the sequence length of the input words, the number of sentences in a single input to the system (batch size), etc. Often wrong initialization can cause the NLP model to crash, produce unexpected outcomes, etc.
	\item \textbf{Logic Bug:} Bugs can occur due to logical errors in the model and the code
	structure. 
	\item \textbf{Processing Bug:} These bugs are related to the wrong choice of the algorithm. 
\end{enumerate}
\textbf{Non-Model Structural Bug (NMSB).} Any bugs (except data and API bugs)
initiated outside the model are classified as ``non-structural bugs''. The sub-categories are the same as structural bugs. However, we only find initialization-related bugs in this category.

==> nlp (Version 920)/challenges.tex <==
\section{Discussion}
\label{sec:challenges}
\paragraph{Black Box Analysis.}
\label{subsec:blackbox}
Although dataset are generally available to the developers, most ML models are black-box in terms of the learning process and model structures. Language models are not an exception. Even though the model functionalities are accessible, the implementation details are hidden inside the model structure. If we think of the language model as a monolithic block, then certainly abstraction has been created to provide controllable parameters to the developers and make changes at a small scale. This is similar to extending a class and change the public section of the parent class. It hides the details of the underlying algorithms from the users. For instance, a developer wants to build a language model for Khmer' language~\cite{blackbox2}. Due to the unavailability of the underlying architecture or the actual dataset used to train \bert, the developer
is finding it difficult to alter the task.
%\begin{figure}[!htp]
%	\includegraphics[scale = .4, width=\linewidth]{blackbox2.png}
%	\caption{Developer Facing Difficulty in Understanding Underlying Impletation.~\cite{blackbox2}}
%	\label{fig:blackbox}
%\end{figure}
Here, from a developer's perspective, an in-depth analysis of each of the layers and the dataset will help to come up with a better understanding of the changes that need to be done. 


%In general, abstraction means creating an interface around a code
%that will hide the implementation level details and give the developers only
%what they need for task-specific implementation. If we think of the language
%model as a whole single, monolithic block, then certainly abstraction has been
%created to provide controllable parameters to the developers and make changes
%at a small scale. This is similar to extending a class and change the public
%section of the parent class. It insulates users from the detailing of the
%underlying algorithm. 
%
%Each language model is capable of performing specific downstream tasks. The
%reason to create this abstraction is that such vast language models are not
%readily understandable. For such scenarios, these models are like clean
%interfaces with specific system functionalities available for the developers
%even though the interface is accessible by the users; however, the
%implementation details are hidden inside the black box. 
%
%Since the state-of-the-art result is achievable using these language models on
%the mentioned dataset along with a set of hyper-parameters. When we use a
%framework for implementing a certain task, at the core level, we are creating a
%mapping from such tasks to a lower level of functionality. So, an in-depth
%analysis of the functionalities of each of these modules or interfaces will
%help the developers to further granulate their understandings of the methods
%and modify them as per their requirements. However, because of the complex
%architecture of these language models, analysis becomes a cumbersome task. 
%
%So the question is, when such conflicts arise? Conflict arises when a developer
%wants to change certain attributes of the pre-defined language models as per
%their need like in Figure \ref{fig:blackbox} shows that how a developer is
%facing issue for all such words that can be written using abbreviation like
%'Could replace with Cud' While performing sentiment analysis as a downstream
%task, the critical words driving the sentiment should be 'better'; however,
%maximum attention score has been given to '\#\#i,' which has no significant
%contribution to sentiment analysis. Here, from a developer's perspective, an
%in-depth analysis of each of the layers along with the shared interfaces will
%help them to come up with a better distribution of scores. 

%\paragraph{Scalability and the Impact on Environment.}
%%If a model is trained at a small scale, however, if the same is used for
%%large-scale implementation, then it outputs considerable accuracy with minimal
%%compromise. Even though trained on a small corpus in a specific environment,
%%the same model will make the best utilization to learn when implemented for
%%large corpus and diverse backgrounds. Then we will say that the model is
%%scalable.
%
%Language models are trained on an enormous corpus, and each of them is specialized for performing certain tasks. For instance, Google has a multilingual model (\textit{mBERT}), trained on a corpus of 104 languages. In the past few years, we have seen an impressive performance from BERT models trained on a specific language however extension of the model to support multi-languages is an example of scalability. However, ~\citeauthor{wu2020all}~\cite{wu2020all} showed that \textit{mBERT} performs better for languages that have large resource availability but perform poorly for small resource languages. Similarly, \roberta, a language model, is developed using improved version of hyper-parameters and increased dataset in comparison to \bert. However, when we consider scaling a model, then it should not be considered only in terms of increasing the architectural size to upgrade the performance. Prior works~\cite{jiao2020tinybert, sanh2019distilbert} have shown that down-scaling the language model has given effective and considerable performance on multiple tasks and natural language dataset.



%However, X~\etal discussed that
%\bert models are not scalable in the sense that not many parameters or the white-box section in the whole learning pipeline. Due to this such restrictions often, a new model is needed to perform a little better with changing the structure of the problem. For example, the \roberta is a model that builds on top of the \bert with X, Y, Z addition.
%Mohna: add X, Y , and Z

%Scalability of the language models has a direct relationship with environmental impacts making it important for the developers to re-examine and re-validate the design process. Recently, it has been noticed that the cost of training model has a direct impact on the environment.  Instead of rebuilding the models to add more data or changing the structure of the model, more scalability should be added so that the current version of the models can be applied for more tasks rather than creating a new one.


\paragraph{Library support and incompatibility}
\label{subsec:scalability}

Most of the pre-trained models have been implemented from emerging research results. A few of them are available through popular deep learning libraries such as \tensor and \torch. However, the core model implementations are still in active development. API structure for the models are often pre-configured with
specific requirements, which resulted in many API and structural bugs. Developers often fail to capture the tight specification from usage examples and documentation. In addition, NLP tasks also need a number of data and platform-specific steps, which are not supported by the pre-trained models locally. For example, to build a sentiment classifier on new dataset using \bert, developers would need to prepare data using external libraries such as \textit{pandas}, \textit{NumPy}, etc., and set up GPU training backend using \tensor, and so on. Therefore, several
dependencies among libraries occur, which are implicit in many cases, causing fatal bugs for the developers. Therefore, there is an immediate need to address the specification and dependency issues by the library developers and researchers. 




==> nlp (Version 920)/classification.tex <==
\subsection{Classification Strategy}
\label{subsec:classification}
Here, we classify the bugs into their types (bug-type), what is causing the bug (root cause), and how the bug affects the system (impact). We define the classification scheme based on prior works~\cite{islam2019comprehensive, zhang2018empirical, beizer1990software} and follow the open coding scheme for each category. 
First, a pilot study has been conducted to identify the need for a new category, and if needed, it has been approved in the discussion among the raters. For impacts and bug types, we found that the classification scheme proposed by \citeauthor{islam2019comprehensive}~\cite{islam2019comprehensive} and \citeauthor{zhang2018empirical}~\cite{zhang2018empirical} are sufficient to address bugs found in NLP-based systems. 
For root cause, we adapted the classification scheme proposed by \citeauthor{islam2019comprehensive} and added new root cause kinds based on the open coding approach. We have added five main kinds and several sub-kinds within that. The entire classification scheme has been shown in \fignref{taxo}.

\textbf{Labeling}. We label the bug-related issues based on the classification scheme fixed in the previous step. The first and second authors independently labeled the bugs. To measure the raters' agreement, we compute the Cohen's Kappa co-efficient~\cite{viera2005understanding} for each 10\% of issues. After two rounds, the Cohen's kappa coefficients for all three categories were $>0.85$, which indicates the perfect agreement. The first and second authors then labeled independently and resolved any disagreement based on discussions.  

%\subsubsection{Overview}
%\label{subsub:overview}
%Before diving into the bug classification scheme, we will briefly discuss standard components involving reusing a pre-trained model. Broadly, NLP model reuse includes (1) data preprocessing and (2) updating the model parameters. The data preprocessing can be done on the training data of the pre-trained models or the domain-specific dataset. Whereas to tailor the model to fit the domain, developers often change the model parameters.
%\subsubsection{Types of Bugs}
%\input{bugtype.tex}
%\subsubsection{Root Cause of Bugs}
%\label{subsubsec:root}
%\input{root.tex}
%\subsubsection{Impacts of Bugs}
%\input{impact.tex}




==> nlp (Version 920)/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}
%% > original
%With the increase in the popularity of the NLP domain, developers are facing several bugs while reusing the pre-trained models. In this study, we mined 9420 issues from 10 repositories of well-known pre-trained models. Furthermore, we filtered these issues into 865 bugs and manually studied them to understand the common bug type, root causes, and impacts. We built a classification scheme based on an open coding scheme and found that the root causes of the bugs are significantly different from the traditional machine learning or deep learning bugs. Our findings can help both NL and SE communities to guide through the most prevalent problems while reusing these models and build an automated repairing approach to address the same. First, we found that large models are bug-prone and have a negative effect on the environment. Building smaller and granular models can help to fix this issue. Second, with the limited choice of control over the reusability, wrong settings can make the system vulnerable to outside attacks. A parameter tuning and validation-based approach could be helpful to increase the robustness of the system. Other major findings include the propagation of the input bias to the output, loss of semantic preservation in the system, etc. By implementing proper specifications to verify the system, semantic preservation, bug propagation could be avoided. 

With the increase in the popularity of the NLP domain, developers are facing several bugs while reusing the pre-trained models. In this study, we mined 9214 issues from 11 repositories of well-known pre-trained models and identified 984 bugs. Then, we manually studied them to understand the common bug type, root causes, and impacts. We built a classification scheme based on an open coding scheme. We determined that the root causes of the bugs are significantly different from the bugs found in traditional deep learning. Specifically, we found that large models are bug-prone and cause memory-related issues. We identified that a parameter tuning and validation-based approach could be helpful to increase the robustness of such systems. We also identified bugs related to the propagation of input bias to the output, loss of semantic preservation in the system, etc. Lastly, we suggest different ways to prevent such issues (i.e., verify the system to ensure semantic preservation, etc.). Our findings can help guide both the NL and SE practitioners and researchers through the most prevalent problems of reusing these models and help build automated repairing approaches to address the same.



% NLP pre-trained models, e.g., \bert , \roberta , \gpt, have shown much success in the recent past. Because of the large size and complex computational needs, developers often face unique challenges while leveraging these models for solving various NLP tasks. 
% In this paper, we studied different types of bugs, their root causes, and impacts occurred while reusing NLP pre-trained models. We mined more than nine thousand issues from GiHub repositories of ten models and filtered 865 bugs. by studying those bugs, we created a classification of NLP bugs and root causes. We reported a number of new bug patterns that developers experienced. Moreover, we suggested a few areas where the models lack usability, functionality, and robustness. The study also showed further research opportunities to employ software engineering techniques to identify and localize bugs in NLP models.

==> nlp (Version 920)/data.tex <==
\section{Study Design}
\label{sec:method}
Here, we describe the methodology to collect the dataset and build
the classification scheme. First, we discuss the data collection steps. Then, we discuss our
classification scheme and labeling approach.
\subsection{Data Collection}
\label{subsec:data}

Figure~\ref{fig:datacollection} shows the data collection steps for selecting the pre-trained models, mining issues from corresponding \gh repositories, and identifying bugs through manual investigation. 

% The first two sentences of this paragraph are not well connected. The transition from the popular open-source... to Huggingface is to abrupt
\textbf{Model Selection.} First, we identify the popular open-source NLP pre-trained models and issues corresponding to that. We start by identifying the list of available pre-trained models. For that, we refer to \textit{Huggingface	Transformers}~\cite{wolf2020transformers, transformer}, an open-source framework that maintains an NLP model hub~\cite{modelHub}. It contains
pre-trained models for various NLP tasks such as text classification, translation, etc. Huggingface Transformers is supported by the most popular deep learning libraries (i.e., \tensor, \torch). Furthermore, several major organizations, including Google, Facebook, Microsoft, Allen Institute, and others, use this framework. However, the issues reported in the
\textit{Huggingface Transformers} are related to problems faced by developers that correspond to the bugs in their platform rather than bugs encountered while using pre-trained models. To focus our study on the bugs that developers face while reusing the pre-trained model, we study the issues reported in the repositories corresponding to each such model. As of January 2022, \textit{Huggingface Transformers} listed 93
pre-trained models in their documentation~\cite{transformer}. Among these models, we found that 36 pre-trained models are open-source and have a \gh repository. Since we aim to identify the bugs developers face while reusing these models, we focus on the issues logged by developers in the \gh. Some of these repositories have very few issues since they do not maintain or update the repository based on discussions and reported bugs. Hence, we filter out the repositories having $ \le 50$ issues (open + closed issues). Based on these criteria, we identified 24 repositories. Finally, to focus on the quality repositories (popularity among developers) and keep our manual analysis manageable, we focus on the repositories with at least 2000 stars~\cite{borges2016understanding}. Thus, we found repositories that correspond to 11 NLP pre-trained models. The number of issues for these models ranges from 76 to 3214 and a total of 9214. We further filtered them to identify bugs in these models.
The details of each such model are given in Table~\ref{tbl:dataset}. 
%
%\textbf{\albert:}~\cite{albert} A Lite BERT is an improvement over \bert , is trained on multiple NLP datasets, with fewer parameters. 
%
%\textbf{\bart:}~\cite{bart} BART is based on a standard transformer architecture used for neural machine translation. It has both an encoder and a decoder. It uses a noisy source text as input and eventually uses a language model for reconstructing the original text by predicting the replacement of noisy tokens.
%
%\textbf{\bert:}~\cite{bert} Bidirectional encoder representations from transformers is based on the transformer architecture. It is pre-trained over a lot of unlabeled textual data to learn a language representation to fine-tune for specific machine learning tasks.
%
%\textbf{\ctrl:}~\cite{ctrl} Conditional Transformer Language Model  is trained on 140GB of text data. It is trained to conditions on control codes that control the content, style, and task-specific behavior.
%
%\textbf{\gpt:}~\cite{gpt2} Generative Pre-trained Transformer-2 is trained on millions of webpages. It is a 1.5 billion parameter transformer-based model that outperforms prior models on 7 out of 8 language modeling datasets.
%
%\textbf{\roberta:}~\cite{roberta} Robustly Optimized BERT Approach is a retraining of BERT with improved training methodology and data.
%
%\textbf{\tf:}~\cite{t5} Text-to-Text Transfer Transformer model is a large neural network model, trained on a mixture of unlabeled text and labeled data from several downstream tasks.
%
%\textbf{\txl:}~\cite{txl} Transformer-XL model, based on Transformer architecture, allows language understanding beyond a certain length without disturbing the temporal coherence, unlike traditional transformer.
%
%\textbf{\xlm:}~\cite{xlm} XLM is an improved version of BERT that achieves better performance in both classification and translation NLP tasks.
%
%\textbf{\xlnet:}~\cite{xlnet} XLNET is a generalized version of \txl. It is based on a large bidirectional transformer that uses larger data. It outperformed \bert on 20 language tasks.
%

\input{datatable.tex}

\textbf{Issue Mining.} Once we fixed the models under study, we mine the
issues related to the \textit{bug} and \textit{bug-fix}. To mine such issues, we
utilize the techniques applied by Garcia~\etal~\cite{garcia2020comprehensive}.
In this approach, the issues with these keywords in the title or body are selected:
\textit{fix}, \textit{defect},
\textit{error}, \textit{bug},
\textit{issue}, \textit{mistake}, \textit{incorrect}, \textit{fault}, and
\textit{flaw}. In addition, the issues labeled as a \textit{bug} by the respective repository are also selected. On top of that, we
remove the issues that are labeled as \textit{wontfix}, which are
primarily not bugs, and there is no fix needed for those issues. Finally, we
identified 1227 issues from \gh out of 9214 issues present in all ten
repositories.

\textbf{Bug Identification.} Once we mine all the bugs-related issues
based on the keyword searching, two raters (first and second authors)
manually went through the issues to mark them as \textit{``bug''} or
\textit{``not bug''}. If there is a discrepancy while labeling the issues, it has been clarified based on the discussion among raters. Finally, 954 
bug-related issues are identified from 1227 issues. Within
these 954 issues, 30 bug-related issues have more than one bug in a single issue.
For such scenarios, we counted them as more than one bug. 
%The labeled dataset can be found in our replication package \cite{}.


==> nlp (Version 920)/datatable.tex <==
\begin{table*}[!htp]
	\centering
	%\vspace{5pt}
	\setlength{\tabcolsep}{2.2pt}
	%\rowcolors{2}{gray!25}{white}
	\footnotesize
	\begin{tabular}{|p{2.4cm}|p{1.1cm}|c|c|c|p{9.8cm}|c|}
		\hline
		\rowcolor{gray!50}
		\multicolumn{1}{|c|}{\textbf{Model Name}}     & \multicolumn{1}{|c|}{\textbf{Owner}} & \textbf{\#Issue} & \textbf{\#Mined}  & \textbf{\#Bugs}  & \multicolumn{1}{|c|}{\textbf{Description}}  & \textbf{Parameters}     \\
		\hline
		\hline
		ALBERT~\cite{albert, lan2019albert} & GR        & \textbf{171}     & \textbf{64}   & \textbf{53}   & A Lite BERT is trained on multiple datasets, with fewer parameters than \bert.& 223M \\
		\hline
		Bart~\cite{bart, lewis2020bart} & FR         & \textbf{3214}    & \textbf{156}  & \textbf{119} & BART is based on a standard transformer architecture used for neural machine translation. It has both an encoder and a decoder. & 406M \\
		\hline
		Bert~\cite{bert, devlin2019bert}     & GR      & \textbf{1091}    & \textbf{299}  & \textbf{216}  & Bidirectional Encoder Representations from Transformers is a transformer architecture-based model. It has been trained over a lot of unlabeled textual data. & 340M\\
		\hline
		CTRL~\cite{ctrl, keskarCTRL2019}  & Salesforce          & \textbf{76}      & \textbf{33}   & \textbf{27} & Conditional Transformer Language Model  is trained on 140GB of text data. &1.6B\\
		\hline
%		Deit~\cite{xlnet, yang2019xlnet}  & FR        & \textbf{120}     & \textbf{40}   & \textbf{20}  & XLNET is a generalized version of \txl. It is based on a large bidirectional transformer that uses larger data. It outperformed \bert on 20 language tasks.& 340M \\
%		\hline
		GPT-2~\cite{gpt2, radford2019language}  & Open AI        & \textbf{232}     & \textbf{89}   & \textbf{70}   &Generative Pre-trained Transformer-2 is trained on millions of webpages.  & 1.5B
		\\
		\hline
		GPTNeo~\cite{gptneo, gao2020pile}  & EleutherAI        & \textbf{138}     & \textbf{78}   & \textbf{44}  & GPTNeo is a transformer based model trained on 825GiB English text corpus.& 2.7B 
		\\
		\hline
		RoBERTa~\cite{roberta, liu2019roberta} & Facebook      & \textbf{3214}    & \textbf{190}  & \textbf{155}  & Robustly Optimized BERT Approach is an improved version of \bert with more data. &355M \\
		%TO-DO:What is the improved methodology?
		\hline
		T5~\cite{t5, 2020t5}   & Google AI          & \textbf{374}     & \textbf{147}  & \textbf{150}   & Text-to-Text Transfer Transformer model is a large neural network model, trained on a mixture of unlabeled text and labeled data from several downstream tasks. & 11B\\
		\hline
		Transformer-XL~\cite{txl, dai2019transformer}& Google CMU & \textbf{128}     & \textbf{35}   & \textbf{19}  & Transformer-XL model, based on Transformer architecture, allows language understanding without disturbing the temporal coherence unlike traditional transformer. & 257M\\
		%TO:DO The sentence does not make any sense
		\hline
		XLM~\cite{xlm, lample2019cross}    & FR       & \textbf{320}     & \textbf{106}  & \textbf{84}  & XLM is an improved version of BERT that achieves better performance in classification and translation-related tasks.& 500M\\
		\hline
		XLNET~\cite{xlnet, yang2019xlnet}  & Google CMU        & \textbf{256}     & \textbf{80}   & \textbf{47}  & XLNET is a generalized version of \txl. It is based on a large bidirectional transformer that uses larger data. It outperformed \bert on 20 language tasks.& 340M \\
		\hline
		\hline
		
		\multicolumn{2}{|l|}{\textbf{Total}} & \textbf{9214}    & \textbf{1277} & \textbf{984}  && \\
		\hline
	\end{tabular}
\vspace{12pt}
\caption{Dataset description -- Pre-trained NLP models. GR: Google Research, FR: Facebook Research.}
\label{tbl:dataset}
\end{table*}

==> nlp (Version 920)/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\begin{enumerate}
   %% this sentence doesn't make sentece >> 
    \item Since NLP tasks require models trained on very large corpus, reusability, replicability and modular software engineering are immediately required. 
    %% <<
\red{
   \item NLP pre-trained models usage is still in its infancy. The models we studied are under active development. Continuous improvement and maintenance of the models require a unified framework and methodologies. 
  \item Our study shows many opportunities to identify the bugs automatically by static analysis. 
  \item Many of the bugs can be fixed by automated repairs. We need more repair tools that leverage both static and dynamic analysis. Furthermore, the interaction between data and model should be made more explainable. 
  \item Finally, the black-box nature of pre-trained models is the reason for many bugs in the client code. The usability of the APIs is also bug concern. More research is needed to enhance the software architecture and design of the NLP models.
  }
\end{enumerate}

==> nlp (Version 920)/impact.tex <==
%Here, we discuss the impacts of the bugs.

\textbf{Bad Performance.} 
Developer often finds that the model is not performing adequately. Such bugs are classified into this category.
%This kind of effect is frequent in NLP-related
%tasks. Reusing or retraining the pre-trained models often cause a drop in
%performance due to several reasons, e.g., dataset not compatible with the type
%of tasks that a model could perform, wrong parameters that hinder the learning
%processes, etc. Due to the large architecture and its opaque computation, minor bad performance is often not observed by the developers. 

\textbf{Crash.} When a program exits with an error, the effect of the bugs
is classified under this category. 
%A program in NLP can halt due to the wrong
%use of execution platform, improper use of pre-trained models, or even the
%wrong structure of data.

\textbf{Data Corruption.} If the output data has been changed unexpectedly, then data corruption occurs. 
%These bugs
%can either be identified by the compiler if it exhibits functional error, otherwise, it is difficult to locate.

\textbf{Hang.} If a program does not return output for a
stipulated time and keeps running, then it generally enters the
hanging state.

\textbf{Incorrect Functionality.} Often, due to a bug in the NLP system, the output of the program is different from the expected behavior.

\textbf{Memory Out of Bound.} Often, a program in NLP halts due to the
unavailability of the memory.
% and this genre of effects is very frequent due to
%the massive size of the models and data. In many cases, the proper partitioning and use of existing memory nodes are not utilized which result into memory out of bound.
%\paragraph{Support Failure}
%The pre-trained models might fail in a specific processing environment or some
%functionality can be still not developed. The lack of testing and robustness in
%the pre-trained models can result into failure for a new task or data property.
%





==> nlp (Version 920)/introduction.tex <==
\section{Introduction}
\label{sec:intro}
``Hey, Alexa! How is the weather outside?'', ``Hey, Google! Play my favorite
song'', or ``Hey, Siri! Set the alarm at 6 pm?'' these are a few
examples in which Natural Language Processing (NLP) has been used in our daily lives. In each one, human speech is transformed into machine-level representations.
\begin{figure}[t]
	\centering
	\includegraphics[width=0.97\linewidth]{rq1processing}
	\caption{An example of NLP reuse-related bug ~\cite{processing}}
	\label{fig:rq1process}
\end{figure}
The
pre-trained networks analyze the inputs and generates results. Over the last decade, there has been extensive work on processing
natural language and an increasing uptick in usage of these models in both
industries~\cite{devlin2019bert, radford2019language, lample2019cross} and
academia~\cite{vaswani2017attention, tensor2tensor, wolf2020transformers}.
%
%NLP is a sub-domain of artificial intelligence that studies how to enable
%machines to understand, interpret, and make predictions on free-form text or
%speech. NLP has received a lot of attention and gained success in many tasks, i.e., sentiment analysis~\cite{groh2011characterizing}, automated
%chatbot~\cite{xu2017new, hu2018touch}, topic modeling~\cite{peinelt2020tbert,
%	lan2019albert}, and more. 
\begin{figure*}
	\centering
	\includegraphics[,trim={12cm 0cm 12cm 0cm},width=.7\linewidth]{NLP.pdf}
	\caption{Data collection steps for studying bugs in NLP pre-trained models}
% 	\vspace{5pt}
	\label{fig:datacollection}
\end{figure*}
However, NLP models require more training
data~\cite{bender2021dangers} and extensive
computation~\cite{strubell2019energy}, compared to other deep learning (DL)-based
models. The additional computation cost requirements led to the development
of several pre-trained NLP models~\cite{devlin2019bert, radford2019language,lample2019cross} that can be reused with minimal changes.
%When compared to other ML domains, practitioners have made extensively applied model reuse in NLP. 
The extensive reuse of NLP pre-trained models helped many developers implement their desired applications efficiently~\cite{lan2019albert, lewis2020bart, keskarCTRL2019, liu2019roberta}, but the black-box nature of the model often leads to software issues and bugs. 
For example, Figure~\ref{fig:rq1process} shows an issue in which a developer was
fine-tuning a multi-lingual \bart~\cite{bart} model to translate sentences from Spanish to English~(\circled{1}). However, for short sentences, the model is producing output in the Arabic language (\circled{2} and~\circled{3}). Since the developers often do not know the internal processes of the pre-trained model, localizing these issues are challenging. 
%Similarly, there are many other issues that developers face when reusing these black-box models. 

There is a vast body of works on understanding the bugs, their root causes, and the
challenges faced by DL~\cite{islam2020repairing,islam2019comprehensive,zhang2018empirical} and machine learning~\cite{thung2012empirical, humbatova2020taxonomy} developers. These works facilitate bug detection, localization~\cite{wardat2021deepdiagnosis, wardat21deeplocalize, nikanjam2021automatic}, and suggest repair strategies~\cite{, zhang2021autotrainer} to practitioners.
However, these studies are mostly done to characterize bugs developers face while building models from scratch, not while reusing pre-trained models. We found that the dataset shared by ~\citeauthor{islam2019comprehensive}~\cite{islam2019comprehensive} has only 16.18\% and 33.57\% of the
DL bugs from \sof and \gh, respectively, are related to reusability. Moreover, the reusability in the prior work's dataset is limited to the image-related models, e.g., ResNet, ImageNet, and are not related to NLP.
In contrast to the prior works, we understand how the bugs introduced while reusing the NLP models are different from the traditional DL bugs and characterized them into the type, root cause, and impact to facilitate further studies. 
%We conducted an
%empirical study on the bugs found while reusing NLP pre-trained models and
%reported the bug types, their root causes, and impacts. 
In this context, we
consider a bug to be caused by reusing the pre-trained models if (1) the bugs
were present in the reused model and propagated to the code while reusing, and/or (2)
bugs found while adapting the pre-trained model by altering code.

%To-Do: Shorten the figures

In this study, we curated the 11 most popular NLP
pre-trained models from a model hub, \textit{Huggingface
	Transformers}~\cite{transformer}. Then we mined 9,214 issues from the \gh
repositories of these models that use these pre-trained models. 
We further filtered the issues that report bugs. After manual checking, we
identified 954 issues that contained 984 bugs introduced while reusing NLP models.
We adapt the classification scheme from a prior work~\cite{islam2019comprehensive} to characterize deep learning bugs and update it based on the open-coding scheme. We answer the following research questions: 
\begin{itemize}[leftmargin=*]
	\item \textbf{RQ1 (Bug Types):} What kind of bugs are prevalent while reusing NLP models, and how do they differ from DL software?
	% \begin{enumerate}
	% 	\item How bugs related to wrong initialization are different from traditional DL bugs?
	% 	\item How are bugs related to the underlying algorithm different from the traditional DL bugs?
	% \end{enumerate}
	\item \textbf{RQ2 (Root Causes):} What are the root causes of the bugs?
	\begin{itemize}
		\item How do the updates in the pre-trained models introduce bugs?
		\item Which NL configuration parameters are causing the models to be bug-prone?
	\end{itemize}
	\item \textbf{RQ3 (Impacts):} How do the bugs impact the NLP software?
\end{itemize}

%- \textbf{RQ1 (Bug Types):} What kind of bugs are common while reusing NLP models?
%
%- \textbf{RQ2 (Root Causes):} What are the causes of the bugs?
%
%- \textbf{RQ3 (Impacts):} How do the bugs impact the NLP software? 

We found several frequent bug patterns that include the wrong update of the models, API misuse, architectural issues, or domain-specific confusion. The key findings
of the paper are as follows:
\begin{enumerate}[leftmargin=*]
	\item Reused NLP models suffer more initialization and memory-related bugs
	than the traditional DL models due to the larger model size. We identified that the average number of parameters and dataset size for the largest DL (ResNet1100, VGG16) models are ~80 million and ~100GB, respectively. Whereas, in NLP (CTRL, T5), it is ~7 billion and ~650GB, respectively, which are significantly large compared to the DL models.  
	\item Traditional DL models are barely reused in production and focus more on data. Whereas, in NLP, the focus is on setting correct parameters (32.3\% of the total bugs) as users often do not have access to the training data of the reused model. 
	\item Due to the black-box nature of the reuse, NLP developers often do not clearly understand the underlying architecture of these models.
	We found that such bugs are seen 14.9\% of the time in NLP, but for DL, it has been seen for 6.3\%.
%	\item Lack of specification in the NLP-based models can cause the input bias to
%	be propagated to the prediction.
\end{enumerate}

\textbf{Outline:} 
%The rest of the paper is organized as follows:
%\secnref{sec:nlp} introduces the
%NLP workflow and the role of pre-trained models. 
In \secnref{sec:method}, we discuss data collection and labeling methodology. \secnref{sec:rq1}, \secnref{sec:rq2}, and \S\ref{sec:rq3} describe the frequent bug types, the root causes of the bugs, and  the common
impacts, respectively. \secnref{sec:related} describes the related works, \secnref{sec:threat}
explains the threats to validity, and \secnref{sec:conclusion} concludes.


==> nlp (Version 920)/macro.tex <==
%\usepackage[table]{xcolor}
%\usepackage[svgnames]{xcolor}
%\usepackage[round]{natbib}
\usepackage{multirow}
\usepackage{rotating}
\usepackage{booktabs} % For formal tables
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage[belowskip=-12pt]{caption}
%\usepackage{subcaption}
\usepackage{rotating}
\usepackage{tabularx}
%\usepackage{subfig}
\usepackage{wrapfig}
\usepackage{listings}
\usepackage{color, colortbl}
\usepackage{balance} % to balance the bibliography
\usepackage{lscape}
\usepackage{hyperref}
\usepackage{xspace}
\usepackage{framed}
\usepackage{syntax}
\usepackage{enumitem}
%\usepackage{hyperref}
%\usepackage{mdframed}
%\usepackage[framemethod=TikZ]{mdframed}
\usepackage{soul}
\usepackage{flushend}
\usepackage[tikz]{bclogo}
% loads also »colortbl«
\usepackage{makecell}
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.92}
\definecolor{Gray}{gray}{0.1}
%\rowcolors{2}{gray!25}{white}
\lstdefinestyle{mystyle}{
	backgroundcolor=\color{backcolour},   
	commentstyle=\color{codegreen},
	keywordstyle=\color{magenta},
	numberstyle=\tiny\color{codegray},
	stringstyle=\color{codepurple},
	basicstyle=\scriptsize,
	breakatwhitespace=false,         
	breaklines=true,                 
	captionpos=b,                    
	keepspaces=true,                 
	numbers=left,                    
	numbersep=5pt,                  
	showspaces=false,                
	showstringspaces=false,
	showtabs=false,                  
	tabsize=2
}

%\definecolor{diffstart}{named}{Grey}
%\definecolor{diffincl}{named}{ForestGreen}
%\definecolor{diffrem}{named}{OrangeRed}

\lstdefinelanguage{Pythonna}{%
	language     = python,
	morekeywords = {to_categorical, flow_from_directory,pad_sequences,load_image},
	morecomment=[f][\color{diffstart}]{@@},
	morecomment=[f][\color{diffincl}]{+\ },
	morecomment=[f][\color{diffrem}]{-\ }	
}

\lstdefinestyle{customc}{
	belowcaptionskip=1\baselineskip,
	breaklines=false,
	frame= single,
	%numbers = left,
	breaklines = true,
	xleftmargin=\parindent,
	language= Pythonna,
	showstringspaces=false,
	%basicstyle=\footnotesize\ttfamily,
	keywordstyle=\bfseries\color{green!40!black},
	commentstyle=\itshape\color{purple!40!black},
	identifierstyle=\color{blue},
	stringstyle=\color{codegreen},
	backgroundcolor=\color{gray!4}
}


\lstset{style=customc}
\newcommand{\change}[1]{{\color{blue!80!white}\textbf{}~#1}\xspace}
%\usepackage{pdflscape}
\newcommand{\centerhfill}[1][\quad]{\hspace{\stretch{0.5}}#1\hspace{\stretch{0.5}}}
\graphicspath{{./figures/}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\fignref}[1]{Figure~\ref{#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref{#1}}
\newcommand{\secref}[1]{\S\ref{#1}}
\newcommand{\secnref}[1]{\S\ref{#1}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\theref}[1]{Theorem~\ref{#1}}
\newcommand{\lineref}[1]{line~\ref{#1}}
\newcommand{\linesref}[2]{lines~\ref{#1}-\ref{#2}}
\newcommand{\linerefNum}[1]{\ref{#1}}
\newcommand{\footnoteref}[1]{$^{\ref{#1}}$}
\newcommand{\commitcount}{100\xspace}
\newcommand{\totalcommit}{500\xspace}
\newcommand{\etal}{{\em et al.}\xspace}
\newcommand{\albert}{\textit{ALBERT}\xspace}
\newcommand{\bart}{\textit{Bart}\xspace}
\newcommand{\bert}{\textit{Bert}\xspace}
\newcommand{\ctrl}{\textit{CTRL}\xspace}
\newcommand{\gpt}{\textit{GPT-2}\xspace}
\newcommand{\roberta}{\textit{RoBERTa}\xspace}
\newcommand{\tf}{\textit{T5}\xspace}
\newcommand{\txl}{\textit{Transformer-XL}\xspace}
\newcommand{\xlnet}{\textit{XLNET}\xspace}
\newcommand{\xlm}{\textit{XLM}\xspace}


% red color
\newcommand{\red}[1]{\textcolor{red}{#1}}

\newcommand{\code}[1]{{\texttt{\footnotesize{#1}}\xspace}}

\newcommand{\sof}{\textit{Stack Overflow}\xspace}
\newcommand{\caffe}{\textit{Caffe}\xspace}
\newcommand{\ho}{\textit{H2O}\xspace}
\newcommand{\keras}{\textit{Keras}\xspace}
\newcommand{\mahout}{\textit{Mahout}\xspace}
\newcommand{\mllib}{\textit{MLlib}\xspace}
\newcommand{\scikit}{\textit{scikit-learn}\xspace}
\newcommand{\tensor}{\textit{Tensorflow}\xspace}
\newcommand{\theano}{\textit{Theano}\xspace}
\newcommand{\torch}{\textit{Pytorch}\xspace}
\newcommand{\weka}{\textit{Weka}\xspace}
\newcommand{\gh}{\textit{GitHub}\xspace}
\newcommand{\paddle}{\textit{paddle}\xspace}
\newcommand{\wa}[1]{{\color{orange!80!white}\textbf{Who to work on:}~#1}\xspace}
\newcounter{rqs}
\stepcounter{rqs}
\newcommand{\heart}{\ensuremath\varheartsuit~}
\newcommand{\sbug}{\textit{320}\xspace}
\newcommand{\gbug}{\textit{347}\xspace}
\newcommand{\qn}[1]{{\bf{RQ\arabic{rqs}: } \em #1}
	\stepcounter{rqs}
}

\newcounter{NumObservations}
\stepcounter{NumObservations}
\definecolor{shadecolor}{rgb}{.9,.9,.9}




\newcommand{\finding}[1]{%
	\begin{mdframed}[
		backgroundcolor= gray!08,
		linewidth=.2pt,
		linecolor = black,
		roundcorner=2pt,
		skipabove=8pt,
		innertopmargin=5pt,
		innerbottommargin=5pt,
		innerrightmargin=4pt,
		innerleftmargin=2pt,
		leftmargin = 2pt,
		rightmargin = 2pt]%
		\noindent{\textbf{Finding \arabic{NumObservations}}: #1} 
	\end{mdframed}%
	\stepcounter{NumObservations}
}


\newcommand{\findingsold}[1]{
	
	\begin{shaded}
		\vspace{-.85em}
		%\hspace{1.5em}
		\textit{{\bf{Finding \arabic{NumObservations}}}: #1.}\\
		\vspace{-1.75em}
	\end{shaded}
	\stepcounter{NumObservations}	
}


%\newcommand{\finding}[1]{
%	\begin{bclogo}[couleur= Orchid!14, epBord= 1, arrondi=0.1, logo=\bcattention,marge= 2, ombre=true, blur, couleurBord=Orchid!80, tailleOndu=3, sousTitre ={\em #1}]{Finding \arabic{NumObservations} $\Rightarrow$ } 
%		
%	\end{bclogo}
%	\stepcounter{NumObservations}
%}
\newcommand{\findings}[1]{
	\begin{bclogo}[couleur= Orchid!14, epBord= 1, arrondi=0.1, logo=\bctrombone,marge= 2, ombre=true, blur, couleurBord=Orchid!80, tailleOndu=3, sousTitre ={\em #1}]{Finding \arabic{NumObservations} $\textbf{:}$ } 
		
	\end{bclogo}
	\stepcounter{NumObservations}
}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{
		\node[shape=circle,fill,inner sep=1pt] (char) {\textcolor{white}{#1}};}}
\newcommand{\findingold}[1]{%
	\begin{mdframed}[
		backgroundcolor= gray!10,
		linewidth=.2pt,
		linecolor = gray!110,
		roundcorner=2pt,
		innertopmargin=2pt,
		innerbottommargin=0pt,
		innerrightmargin=4pt,
		innerleftmargin=2pt,
		leftmargin = 0pt,
		rightmargin = 0pt]%
		\noindent{\textbf{Rule \arabic{NumObservations}}: #1} \\
	\end{mdframed}%
	\stepcounter{NumObservations}
}
\lstdefinestyle{mystyle}{
	backgroundcolor=\color{backcolour},   
	commentstyle=\color{codegreen},
	keywordstyle=\color{magenta},
	numberstyle=\tiny\color{codegray},
	stringstyle=\color{codepurple},
	basicstyle=\scriptsize,
	breakatwhitespace=false,         
	breaklines=true,                 
	captionpos=b,                    
	keepspaces=true,                 
	numbers=left,                    
	numbersep=5pt,                  
	showspaces=false,                
	showstringspaces=false,
	showtabs=false,                  
	tabsize=2
}

==> nlp (Version 920)/modelUpdate.tex <==
\subsection{How updating the pre-trained models introduce bugs?}
\label{subsec:reuse}
Approximately one-third of the bugs in reusing pre-trained models are related to updating models. Such circumstances are very nominal in traditional DL, with prior work not defining any classification category representing their root causes. In this context, updating a pre-trained model can be done by migrating the model to another system, setting up checkpoints to store intermediate training results, retraining the model with either additional or new data, refining the weight, fine-tuning the model, etc., to match the user's intended functionality with the one provided by the model.

\finding{Majority of the bugs (32.3\%) are caused due to updating the pre-trained models.}

%Pre-trained models can be reused by 1) plugging the model into the software and
%start predicting, 2) updating the dataset to match with the model specifications
%(without retraining the model), e.g., shape, type, etc., and 3) update the model
%by retraining, fine-tuning, asserting checkpoints, refining weights, etc. 
%Here, we discuss how updating models cause bugs in NL software. We found
%that most of the bugs are caused while tailoring the model to the %need of the
%developer. 
% \begin{figure}[!ht]
% 	\centering
% 	\includegraphics[width=\linewidth]{rq2f1}
% 	\caption{Bugs while retraining T5 model~\cite{rq2f1}}
% 	\label{fig:reuse}
% \end{figure}
In an issue reported by a developer~\cite{rq2f1} discusses that re-training a \tf model with a custom dataset and the model produces unexpected
output, generating prefixes in German or Spanish while the model was
trained for the English dataset. This is due to insufficient training. Further investigating, we found
several sub-categories of such bugs, e.g., migrating models and model-related artifacts,
fine-tuning, imposing checkpoints, refining models' weight and bias, and
re-training models with custom datasets and parameters. 
%The distribution of each category w.r.t. the pre-trained models are shown in Table~\ref{tb:reuse}. 
As discussed previously, this phenomenon is unique to the NLP model reusability
as it is not very common to reuse traditional DL models. Most traditional DL models are built from scratch. For instance, only 3.5\% of the models curated (out of 6368 \gh repositories) by \citeauthor{gonzalez2020state}~\cite{gonzalez2020state} are related to reusing pre-trained model. We verify the reuse by identifying the presence of a pre-trained model in the list of import statements, and/or a compiled model is loaded to the
code. We found that most bugs introduced while re-training are due to migrating models, re-training the model, and fine-tuning the models, and we discuss each cause in the paragraphs below.
%To:Do: Sumon: run a query
%With further investigation, we found these bugs can further be classified into
%smaller categories and the distribution of each category for each model has
%been shown in Table~\ref{tb:reuse}. We found that 

%While reusability is widely popular in software engineering domain, it has not
%been widespread in machine learning tasks. However, in NLP, due to the size and
%complexity of the models, training from scratch is often not a feasible
%approach.
%Thus, most of the NLP models are created by large industries, and developers
%craft them based on their needs. However, due to the unavailability of the
%training dataset, and underlying implementations, developers often face issues
%while
%reusing such models. 
%\input{reusetable.tex}
\subsubsection{Migration}
\finding{11.17\% of the bugs are introduced while migrating the pre-trained
	models.}
A majority of the bugs are generated while loading
the pre-trained models and other associated components. The most common
ones are the missing files and the incompatibility between the model and the
input. For instance, an issue~\cite{migration} in
\bert, where a conversion error occurred due to the mismatch between the input
requirement of the pre-trained model and the available APIs, e.g., \tensor.
%Also, the requirement includes JavaScript, but the serialization
%has not been
%defined. 
%These bugs are mostly observed in \gpt , while importing, due to the large
%size.

\textbf{\textit{Implications.}}
%In order to address these migration-related problems, a unified platform would help to provide all the necessary pre-requisites. 
These migration issues are very similar to the software component migration~\cite{plakidas2018software, kum2008autosar, fleurey2007model, choi2004fast,phan2017statistical} problems, where due to ever-changing platforms, paradigms, and techniques, transferring software from one infrastructure to another may cause bugs. However, approaches to resolving such issues~\cite{plakidas2018software, kum2008autosar, fleurey2007model} are limited to the traditional software and currently are not applicable to both DL and NLP-based software. Also, in SE, there have been works on program fragments and linking~\cite{cardelli1997program}. In this particular work~\cite{cardelli1997program}, Cardelli has proposed the notion of the separate compilation of the program fragments and linking them together to form a complete program. The components involved in the migration tasks, e.g., the model, input data, API, can also be compared as program fragments, where each fragment cannot individually be compiled or type-checked. The type-checking only occurs when all the components form the complete program. If the type-checking fails while linking the fragments, then migration-related bugs occur. However, suppose we can enable the separate compilation of the program fragments,  we can identify whether each fragment can safely be linked to other components or fragments. Also, we can validate if certain fragments can be safely replaced with other fragments while migrating to a different environment.  We believe that both research directions could be an interesting avenue to venture into the SE-PL-DL community.
% This stems from the fact that the transformer-based models are still
% being enhanced by researchers and developers from diverse teams. Concrete
% standardization methods and frameworks would benefit the developers to migrate
% between models. 

\subsubsection{Retraining} 
\finding{9.14\% of the all the bugs are related to retraining.} % the pre-trained model
The pre-trained models can be reused (1) without any modification, (2) by re-training
with changing parameters, or (3) by re-training with an additional dataset. In this
section, we discuss the second and third approaches of reusing pre-trained
models.
Re-training without new data can be achieved when a model $M$ is trained on a dataset $D$ and has been further trained with a different set of initialization
parameters. Prior research~\cite{song2020information, zanella2020analyzing} has found that retraining increases the chance of information leakage as the dataset is not evolved during the process. So, if an adversary receives certain information about the dataset, the NLP model can easily be attacked by perturbing the words~\cite{zhang2021red}.
% \begin{figure}[!htp]
% 	\centering
% 	\includegraphics[width=\linewidth]{retraining}
% 	\caption{Model does not learn while retraining~\cite{retraining}.}
% 	\label{fig:retraining}
% \end{figure}

Retraining by addition of dataset is also referred to as incremental
training~\cite{syed1999incremental} \cite{wu2019large} or continuous
learning~\cite{collobert2008unified}. Here, a model $M$ is trained with a dataset
$D$, and re-trained with new data $D'$ to create a model $M'$. For instance,
in an issue~\cite{retraining} logged by developers discussed that while using \bert
model on an example dataset, the accuracy is very low. However, while
predicting, the prediction accuracy is very high (close to 1) for the testing
dataset. To fix the issue, the model requires more training. Since the pre-trained model already has a
certain amount of knowledge, it was sufficient to predict the
examples in the testing dataset, which is essentially smaller than the training dataset. However, it is not sufficient for predicting
examples from the training dataset.

\textbf{\textit{Implications.}}
Developers are often not aware of the differences between different types of
re-training. The focus is more on accuracy than on other aspects, e.g.,
fairness and data leakage. Updating the APIs with the consequences of different
re-training can help developers make better-informed decisions.

\subsubsection{Fine Tuning}
% \begin{figure}
% 	\centering
% 	\includegraphics[width=0.4\textwidth]{finetuning}
% 	\caption{An issue related to finetuning~\cite{finetuning}.}
% 	\label{fig:finetuning}
% \end{figure}
Developers often re-structure the pre-trained models to fit the requirement. For
instance, in an issue reported in \bert~\cite{finetuning}, where the developer modified the model, which mostly includes steps, i.e., pruning the model
changing the parameters. However, it has been noticed that fine-tuning does a negative effect due to the presence
of spelling mistakes. A single
mistake from ``could'' to ``cud'' has changed the prediction result as well as the
attention on the words. Such incidents could also be used as backdoor attacks to the model, where an attacker can knowingly change a single word in such a way that the final outcome of the model has also been changed~\cite{chen2021badnl, yang-etal-2021-rethinking}.
% Also, fine tuning can lead to crashing. For example,
% an issue~\cite{finetune}  reported while reusing \bart describes the difficulty
% faced by the
% developers during fine-tuning. The developer pruned the network, and
% that causes the mismatch of the shape, and the program ends up crashing. 


==> nlp (Version 920)/nltable.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet18'
\begin{table}[htbp]
\centering
\vspace{5pt}
\caption{Distribution of Language Specific Parameters}
\setlength{\tabcolsep}{3pt}
\rowcolors{2}{gray!25}{white}
    \begin{tabular}{|l|r|r|r|r|r|r|r|}
    	\hline
    		\rowcolor{gray!50}
     \textbf{Model} & \textbf{Batch} & \textbf{Token} & \textbf{Lang} & \textbf{ML} & \textbf{Vocab} & \textbf{Sen} & \textbf{Others} \\
    \hline
    \hline
    ALBERT & 9.1\% & 36.4\% & 0.0\% & 9.1\% & 27.3\% & 0.0\% & 18.2\% \\
    \hline
    Bart  & 10.0\% & 25.0\% & 35.0\% & 20.0\% & 0.0\% & 5.0\% & 5.0\% \\
    \hline
    Bert  & 25.7\% & 24.3\% & 14.3\% & 18.6\% & 14.3\% & 2.9\% & 0.0\% \\
    \hline
    CTRL  & 42.9\% & 14.3\% & 0.0\% & 0.0\% & 42.9\% & 0.0\% & 0.0\% \\
    \hline
    GPT-2 & 0.0\% & 0.0\% & 0.0\% & 66.7\% & 33.3\% & 0.0\% & 0.0\% \\
    \hline
    RoBERTa & 0.0\% & 35.3\% & 23.5\% & 5.9\% & 5.9\% & 29.4\% & 0.0\% \\
    \hline
    T5    & 21.4\% & 35.7\% & 14.3\% & 21.4\% & 7.1\% & 0.0\% & 0.0\% \\
    \hline
    T-XL & 20.0\% & 0.0\% & 0.0\% & 40.0\% & 40.0\% & 0.0\% & 0.0\% \\
    \hline
    XLM   & 28.6\% & 7.1\% & 23.8\% & 11.9\% & 26.2\% & 2.4\% & 0.0\% \\
    \hline
    XLNET & 46.2\% & 23.1\% & 15.4\% & 15.4\% & 0.0\% & 0.0\% & 0.0\% \\
    \hline
    \hline
    \textbf{Total} & \textbf{22.8\%} & \textbf{21.8\%} & \textbf{17.3\%} & \textbf{16.3\%} & \textbf{15.8\%} & \textbf{4.5\%} & \textbf{1.5\%} \\
    \hline
    \end{tabular}%
  \label{tb:language}%
\end{table}%



==> nlp (Version 920)/overview.tex <==
\section{Natural Language Processing Systems}
\label{sec:nlp}
\begin{figure*}
	\includegraphics[, width=1\linewidth]{overview.pdf}
	\caption{The Workflow of Reusing Pre-Trained Models for Natural Language
		Processing Tasks.}
	\label{fig:overview}
\end{figure*}
Before we begin the bug-related discussion, we briefly discuss common components involving reusing a pre-trained model. Figure \ref{fig:overview} shows the traditional workflow, which is what most developers follow for reusing models. Broadly, the components are classified into, 1) data
preprocessing, 2) reusing models, and 3) task customization.


\textbf{Data Preprocessing.} 
The data preprocessing can be done on the training data of the pre-trained models or the domain-specific dataset. Since the training dataset is not readily available to the developer while reusing, we consider it as a black box component (grey boxes in Figure \ref{fig:overview}). At this stage, an initial transformation of the free-form text is
performed. The transformation includes tokenization, normalization, removal of %% I feel that the transformation should have all the steps listed here
unwanted segments, etc. These transformations will help attain a better feature representation of the raw data that can be used later. %These transformations 
%will help the raw data for better feature representation

\textbf{Reusing Pre-trained Model.}
At this stage, the pre-trained models are reused in any of the three ways:
\begin{itemize}[leftmargin=*]
	\item Without any change: These models can be reused without any alteration to the input or output. For instance, the GitHub issue discusses how the \bert model can directly be reused.
	\item Transfer learning: In this setting, the model pre-trained on one task is used for a different task. It helps in adding new abilities to the model without having to re-train from scratch.
	\item Fine-tuning: In this setting, the models are re-trained on the domain-specific dataset to capture the task-specific features. In comparison to transfer learning, here, only hyper-parameters are optimized for a specific pre-trained model.
\end{itemize}
%% Consider rewriting the following paragraph and including additional explanation about "the needs"
%% if you start a list with "e.g.," there's no need to put "etc." at the end.
\textbf{Task Customization.} In this stage, downstream tasks, e.g., sentiment 
analysis, opinion mining, information retrieval~(\cite{tang2016aspect,
	rush2015neural}). Broadly, we can categorize the modeling technique either as a single-task or
multi-task model. Single-task models address applications (Task 1, Task 2,
\dots, Task $n$) as independent components, whereas multi-task models address
multi-applications by leveraging synchronization through interfaces between
them. 

==> nlp (Version 920)/parameter.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet12'
\begin{table}[htbp]
%\begin{wraptable}{R}{0.5\linewidth}
	\centering
  \small
	%\vspace{25pt}
	\caption{Pre-trained Models' Description.}
	\setlength{\tabcolsep}{3pt}
	\rowcolors{2}{gray!25}{white}
    \begin{tabular}{|c|c|c|c|}
    \hline
    \rowcolor{gray!50} \textbf{Year} & \textbf{Model} & \textbf{Parameters} \\
    \hline
    \hline
    2019 & \albert & 223M \\
    \hline
    2019 & \bart  & 406M\\
    \hline
    2018 & \bert  & 340M\\
    \hline
    2019 & \ctrl  & 1.6B\\
    \hline
    2019 & \gpt & 1.5B\\
    \hline
    2019 & \roberta & 355M\\
    \hline
    2019 & \tf    & 11B\\
    \hline
    2019 & \txl & 257M\\
    \hline
    2019 & \xlm   & 500M\\
    \hline
    2019 & \xlnet & 340M\\
    \hline
    \end{tabular}%
  \label{tb:modelsize}%
\end{table}%
%\end{wraptable}


==> nlp (Version 920)/related.tex <==
\section{Related Works}
\label{sec:related}

There is a vast body of works in DL bug study~\cite{islam2019comprehensive, islam2020repairing, thung2012empirical, zhang2018empirical, garcia2020comprehensive, humbatova2020taxonomy, wardat21deeplocalize, zhang2021autotrainer, nikanjam2021automatic, schoop2021umlaut, chakraborty2021does, liu2021reproducibility}. Here, we discuss the closest works.

Thung~\etal~\cite{thung2012empirical} have studied three machine learning systems, Apache Mahout, Lucene, and OpenNLP. Bug-type and their severity have
been identified for these systems. Though this dataset has a system
related to NLP, they did not focus on NLP model reusability.

\citeauthor{chen2021empirical}~\cite{chen2021empirical} have studied the deployment faults of DL-based mobile applications using 304 deployment faults from \sof and \gh. They have provided a taxonomy with 23 fault categories and corresponding fix strategies. Whereas we study the bugs while reusing the pre-trained NLP models.

\citeauthor{zhang2018empirical}~\cite{zhang2018empirical} have studied the software built using the \tensor
library. This work is done on 175 bugs found in \sof posts, and \gh
commits. These bugs are classified into symptoms and causes. Though this
work has charted the course in studying DL bugs, the bugs
found in traditional DL libraries are significantly different from
those found while reusing the NLP models. 
%We have studied 10 pre-trained language models in this work and categorized the bugs from bug type, root cause, and impacts. This study has been done independently of the usage of the deep learning library. 

Islam~\etal~\cite{islam2019comprehensive} have studied bugs from five different
DL libraries using 2716 \sof posts and 500 \gh commit. They 
found 415 bugs from \sof posts and 555 from \gh commits. This work
classified the bugs into the root cause, bug type, and effect. Furthermore,
%% different bug stages in the pipeline?
they studied bugs found in different pipeline stages and the presence of
different anti-patterns.
Our classification scheme has been adapted from this work. However, we found that the
NLP-model bugs are significantly different. 

Humbatova~\etal~\cite{humbatova2020taxonomy} have studied 1059 \sof and \gh
codes and developed a taxonomy of the faults seen in these posts and commits. 
This study also focused on traditional DL and did not consider the reusability of models in the NLP domain.


Chakraborty~\cite{chakraborty2021does} has studied 80 \sof posts to determine the type of bugs occurrence when reusing, particularly BERT models. We study the reuse of the 11 popular NLP models. We mined 9,214 issues from \gh and identified 984 bugs. Also, we provide a taxonomy with bug types, root causes, and impacts. 

==> nlp (Version 920)/reusetable.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet19'
\begin{table}[thbp]
	\centering
  \footnotesize
	\vspace{5pt}
	\caption{Distribution of Bugs due to Updating the Pre-trained Models}
	\setlength{\tabcolsep}{3pt}
	\rowcolors{2}{gray!25}{white}
    \begin{tabular}{|l|r|r|r|r|r|r|}
    		\rowcolor{gray!50}
    		\hline
    \textbf{Model} & \multicolumn{1}{c|}{\textbf{Migration}} & \multicolumn{1}{c|}{\textbf{Retrain}} & \multicolumn{1}{c|}{\textbf{Fine Tuning}} & \multicolumn{1}{c|}{\textbf{Checkpoint}} & \multicolumn{1}{c|}{\textbf{Refine Weight}} \\
    \hline
    \hline
    ALBERT & 23.53\% & 47.06\% & 17.65\% & 11.76\% & 0.00\%\\
    \hline
    Bart  & 19.15\% & 29.79\% & 31.91\% & 19.15\% & 0.00\%\\
    \hline
    Bert  & 39.34\% & 18.03\% & 11.48\% & 31.15\% & 0.00\%\\
    \hline
    CTRL  & 50.00\% & 0.00\% & 50.00\% & 0.00\% & 0.00\%\\
    \hline
    GPT-2 & 88.24\% & 0.00\% & 0.00\% & 11.76\% & 0.00\%\\
    \hline
    RoBERTa & 30.91\% & 41.82\% & 18.18\% & 7.27\% & 1.82\%\\
    \hline
    T5    & 13.73\% & 43.14\% & 27.45\% & 15.69\% & 0.00\%\\
    \hline
    T-XL & 50.00\% & 50.00\% & 0.00\% & 0.00\% & 0.00\% \\
    \hline
    XLM   & 62.50\% & 12.50\% & 12.50\% & 6.25\% & 6.25\% \\
    \hline
    XLNET & 44.44\% & 22.22\% & 22.22\% & 11.11\% & 0.00\% \\
    \hline
    \hline \textbf{Total} & \textbf{33.33\%} & \textbf{30.11\%} & \textbf{19.35\%} & \textbf{16.49\%} & \textbf{0.72\%} \\
    \hline
    \end{tabular}%
  \label{tb:reuse}%
\end{table}%


==> nlp (Version 920)/root.tex <==
In this section, we discuss the common root causes of the bugs. First, we discuss all the root causes that we identified, then highlight the most prevalent causes. In Figure~\ref{taxo}, we illustrate all classifications of the root causes, and the blue boxes represent that these bugs are also present in the traditional DL models.


\textbf{Data Faults.}
If the bugs are caused by the incompatibility of the data to the model, we categorize them as data faults.
%For example, in the following code snippet \cite{databugex}, the developers mistakenly passed wrong dimension of data to the Bert model. Fixing line 3 to \texttt{self.bert(sent_id, attention_mask=mask)[:2]}, makes the model work as expected.
%
%\begin{lstlisting}[basicstyle=\fontsize{6}{6}\ttfamily,language = python]
%def forward(self, sent_id, mask):
%   #pass the inputs to the model  
%   _, cls_hs = self.bert(sent_id, attention_mask=mask)
%   x = self.fc1(cls_hs)
%   x = self.relu(x)
%   x = self.dropout(x)
%   # output layer
%   x = self.fc2(x)
%   x = self.softmax(x)
%   return x
%\end{lstlisting}
Bugs in this category can be broadly classified into, 
\begin{enumerate}[leftmargin=*]
	\item \textbf{Type:} These bugs occur due to wrong or mismatched data type.
	\item \textbf{Shape:} Dimension mismatch of input data leads to
	these bugs.
	\item \textbf{Size:} Often, the model expects a predetermined size of the input,
	which can cause these bugs.
	\item \textbf{Unaligned Tensor:} Incompatibility in the data flow of the
	tensors can cause bugs.
\end{enumerate}




\textbf{Algorithmic Error.}
Bugs can occur due to logical or conditional errors such as missing conditions in weight updates, division by zero, etc. The root causes are sub-categorized into,
\begin{enumerate}[leftmargin=*]
	\item \textbf{Logic:} These bugs occur due to
	missing any concept or logic. 
	\item \textbf{Computational Error:} Such bugs appear when existing
	computation produces incorrect results. 
	\item \textbf{Missing Conditions:} If the pre- or post-conditions of any computation
	need to be added/fixed.
\end{enumerate}

%\subsubsection{Configuration}
%Using the pre-trained model require many configurations such as directory
%setup, linking configuration file, setting configuration parameters, etc. Bugs
%can occur because of missing a specific configuration requirement or incorrect
%configuration values.

\textbf{Updating the Pre-trained Model.}
Reusing the pre-trained models often requires satisfying model-specific
requirements. Violating them can introduce bugs in the system. For example, 
\begin{enumerate}[leftmargin=*]
	\item \textbf{Migration:} While migrating pre-trained models to accommodate different
	tasks or datasets, the model requirement does not match with other environments and causes bugs. 
	\item \textbf{Checkpoint:} In DL, creating checkpoint is a common practice during training. This helps one to get intermediate results while performing extensive training. However, we found that often problems may occur while saving these checkpoints or accessing existing checkpoints of the trained model.
	\item \textbf{Re-train :} Bugs introduced while re-training the models on new training data.
	\item \textbf{Refine Weights:} A pre-trained model can offer
	ways to
	refine existing weights. 
	\item \textbf{Fine Tune: }Bug caused while tuning the parameters.
\end{enumerate}

\textbf{Architectural Incompatibility.}
The prebuilt NLP models can have an implicit architectural requirement that poses different
types of incompatibility in the user's system. 
Moreover, the models are resource
hungry and sometimes do not go through exhaustive testing on different
combinations of computational architecture, which causes these bugs. 
The types of such bugs are: 
\begin{enumerate}[leftmargin=*]
	\item \textbf{Memory:} The
	pre-trained models require high memory and often that causes bugs.
	\item \textbf{Concurrency:} Many models allow
	multiple training threads for speedup but cause bugs for strict concurrency assumptions. 
	\item \textbf{Distributed Learning:} Sometimes, these models can be run on the distributed architecture, e.g., multiple cores of CPU or GPU, which leads to bugs.
\end{enumerate}

\textbf{Incorrect Execution Environment.}
Pre-trained models have been made available within different DL packages, e.g.,
\tensor, \torch. 
%Incorrect versions of these frameworks can cause bugs in the
%program. Furthermore, the underlying platform or operating system can also
%cause execution environment bugs. 
The subtypes in this category are:
\begin{enumerate}[leftmargin=*]
	\item \textbf{Cross-platform:} These bugs can occur because of specific requirements of
	the underlying platform, e.g., operating system. 
	\item \textbf{Cross-framework:}
	Incompatible versions of Python or required packages such as \tensor, \torch can be the root cause of this type of bug.
\end{enumerate}


\textbf{API Misuse.}
These bugs can be caused due to, 
\begin{enumerate}[leftmargin=*]
	\item \textbf{Absence of Inter-API Compatibility}:
	There are many API dependencies in the NLP programs, i.e.,
	\textit{Scikit-Learn}, \textit{Tensorflow}. Often these APIs are not compatible in performing a task jointly.
	\item \textbf{API Change:}
	These bugs are related to API versioning.
\end{enumerate}

%Rangeet: Need to fix the above sentence.

\textbf{Confusion in NL-specific Specifications.}
A vast majority of the bugs are due to the missing vocabulary, incorrect sequence length, wrong choice of tokenization mechanism while
preprocessing the data and re-training the model. We further categorized such root causes into the
following categories:
\begin{enumerate}[leftmargin=*]
	\item \textbf{Vocabulary: }Bugs can occur because of
	inappropriate vocabulary or accessing the vocabulary in specific tasks.
	\item \textbf{Tokenization: }When re-training the models on a new dataset, the
	tokens should be preprocessed in accordance with the pre-trained model versions.
	\item \textbf{Sentence: }Often, the semantics and syntax of the sentences differ
	with the customization of NLP tasks, which leads to bugs. 
	\item \textbf{Batch Size: }Because of heavy resource computations and lengthy
	training process, the batch size needs frequent updating, which results in
	NL-specific bugs.
	\item \textbf{Language:} Since different human languages have a variety of structures;
	specific preprocessing and task customization is needed to reuse the pre-trained
	models. In this process, developers can face NL-related bugs.
	\item \textbf{Maximum
		Length: }These models have a hard threshold of the supported maximum length of
	sentences. Developers often need to tune that, which causes bugs.
\end{enumerate}


\textbf{Programming Error.}
These bugs occur due to any other programming issues such as: 
\begin{enumerate}[leftmargin=*]
	\item \textbf{Syntax
		Error:} Bugs might occur due to incorrect syntactical errors such as missing
	punctuations,
	parenthesis, etc.
	\item \textbf{Coding:} Other programming errors such as the wrong loop
	breaking, missing corner cases, misusing variable names, etc. causes bugs in
	the NLP models.
\end{enumerate}

==> nlp (Version 920)/rq1.tex <==
% \section{How Bug Types Are Different from the Traditional DL Software}
\section{What are the prevalent bug types while reusing NLP models}
\label{sec:rq1}


%Motivation for studying this research question.
Here, we discuss the type of bugs found while reusing NLP models.
%Here, we discuss the most common bug types seen while reusing the
%pre-trained NLP models. First, we discuss each type of bugs and then discuss how they are different from the traditional DL bugs.
\input{bugtype.tex}
% the sentence that starts with "Since" and ends with "models" is too long and
%confusing. Consider rewriting it. 
%In prior works~\citeauthor{islam2019comprehensive}~\cite{islam2019comprehensive}, this taxonomy were
%built upon bugs seen in traditional software~(\cite{beizer1990software}).
\subsection{What are the key differences between DL and NLP bug types?}

We found that the bug-type categories proposed by \cite{islam2019comprehensive} are sufficient to represent the bugs seen while
reusing the NLP pre-trained models. However, the distribution, characteristics,
and implications are significantly different. 
Here, we discuss each such category and extend that to highlight the
commonalities and variabilities with the DL bugs. 
\begin{figure}
	\centering
	\includegraphics[width=.95\linewidth]{newBugtype}
	\caption{Classification of bug types}
	\label{fig:bugtypeTaxo}
\end{figure}
%This discussion will help the research community understand the bug categories.
%Also, it will help practitioners design, develop, and improve tools to resolve
%these NLP-related bugs.
%% Is there a common type of API bug that these frameworks have?
\begin{figure*}[!htp]
	\centering
	\begin{subfigure}{.5\textwidth}
		\centering
		\includegraphics[, trim={2cm 7cm 0cm 5cm},width=0.55\linewidth]{bugtype.pdf}
		\centering
		\caption{Distribution of bug types in NLP (labels $<$5.8\% are hidden)}
	\label{fig:bugtype}
	\end{subfigure}%
	\begin{subfigure}{.5\textwidth}
		\centering
		\includegraphics[, trim={2cm 7cm 0cm 5cm},width=0.55\linewidth]{bugtypeDL.pdf}
		\caption{Distribution of bug types in DL (labels $<$3.0\% are	hidden)}
	\label{fig:bugtypeDL}
	\end{subfigure}
	\caption{Comparison between NLP and DL bug types~\cite{islam2019comprehensive} and their distributions}
\end{figure*} 
In Figure.~\ref{fig:bugtype} and \ref{fig:bugtypeDL}, we show the distribution of bugs in NLP-based software and the traditional DL-based software, respectively.
We found that API bugs (26.1\%), initialization bugs (both structural and
non-structural) (31.7\%), and processing bugs (14.9\%) have been observed for more than 70\%
of the bugs in our dataset. Whereas, in the traditional DL, the most prevalent bugs are API bugs (32.6\%), data bugs (17.0\%),
dataflow bugs (15.8\%), etc. 

This suggests that both NLP and traditional DL software are API intensive. We found that versioning (16.02\%), API incompatibility (23.44\%), and execution environment setup (15.63\%) are the most common cause of API bugs. 
% Especially these bugs are seen while reusing \roberta and \tf models. This is mostly because these models are relatively new and are still in development. 
A uniform API definition can help inform the developer about different model reuse. For example, even though Huggingface provides a platform to reuse curated models, they do not provide a unified API specification applicable to different models. Building such unified specifications could help developers to avoid these issues.

We also found that the
dependency on the data for NLP-based software and DL-based software is significantly different. First, a pre-trained NLP
model requires little to no additional data for further usage. Second,
retraining these NLP models is not as data-intensive as training a traditional DL
model from scratch. Here, the majority of
the obstacles developers face are setting the correct model for a problem
(NLP: 14.9\%, DL: 6.2\%) and correctly reusing the model (NLP: 31.7\%, DL: 3.5\%), and such issues rarely occur in the traditional DL-based software. %(processing bugs: 6.2\% and Initialization Bugs: 3.0\%).
%The
%processing bugs mostly take place after loading the model, during fine-tuning,
%or retraining. 
%\begin{figure}[!ht]
%	\centering
%	\includegraphics[width=0.75\columnwidth]{bug-distrib.pdf}
%	\caption{Bug Type Distribution across NLP Models}
%	\label{fig:bugtypemodel}
%\end{figure}
Also, the logic bugs (8.3\%) are not as common as in traditional DL software (18.1\%). The primary reason is that developers often do
not alter pre-trained models' logic. 
%time.
%The overall bug type distribution of the NLP models is shown in Fig.~\ref{fig:bugtypemodel}. 
Next, we discuss some of the key differences.
%Here, we discuss the most prevalent bug types in details.
%We found that setting up or initializing the environment,
%loading a pre-trained model, and executing it on a proper architecture is often
%challenging for developers. 

%\subsection{API Bug}


\subsection{How Initialization Bugs in NLP are Different From Traditional DL Bugs?}
%\textbf{Discuss what is initialization bug and what it looks like in traditional DL}.
One key part of building a model in both DL and NLP-based software is the choice of the parameters, setting up the execution environment, etc. We found that the majority of such problems are due to the massive size of these pre-trained models.
\finding{Larger NLP models introduce more initialization bugs.}
Initialization bugs are prevalent in all models, with a heavy presence in \gpt and \ctrl. 
%In both \gpt and \ctrl, the majority of the NMSB.  
Further investigating, we found that 25.47\% of the bugs in this category originated due to issues while setting up the execution environment. In the traditional DL model, initialization bugs do not occur much (3.29\%).  Since the average size of the DL model is significantly less than that of NLP models, the wrong environmental setup does not affect as much as it does in NLP. We found that for the largest DL models (ResNet1100, VGG16), there are $\sim$80 million parameters, and the size is $\sim$100GB, on average. Whereas, for the same NLP models (CTRL, T5), the average number of parameters and size is $\sim$7 billion and $\sim$650GB, respectively, which is significantly more than the DL models. 
In Table~\ref{tbl:dataset}, the models with their corresponding sizes are shown. To identify the model size, we looked into various versions of the models and listed them according to the total number of parameters. 
%Though the largest
%model in our dataset is \tf; there are five versions of \tf, Small (60M), Base
%(220M), Large (770M), 3B (3B), and 11B (11B), and developers commonly use the
%base version of the model. However, for \ctrl and \gpt, the frequently used
%models are with 1.5B and 1.6B parameters, which is bigger than any other models in
%our dataset (except \tf). 
Due to the large size of the model, loading them to CPU or GPU requires high resources. These bugs cause the abrupt stop of the
execution (66.67\%) and memory issues (13.65\%). Also, Strubell~\etal~\cite{strubell2019energy} identified the resource consumption of the models and their impact on the environment. They found that training a language model emits 6x more $CO_2e$ than a car running on fuel for a year. So, while using the models, the size
should also be taken into account. 
%A unified platform that can suggest
%the model based on the intent (task, dataset, available resources) of the
%developer could help mitigate these bugs and lessen the harmful effect
%on the environment.
%\input{parameter.tex}

\textbf{\textit{Implications.}}
The reuse of pre-trained NLP models is very similar to the software reuse before the notion of modular programming. With finer reuse~\cite{parnas1976design, parnas1972criteria}, parts of the software can be reused and replaced. Recently, for image-based classification problems, \citeauthor{pan2020decomposing}~\cite{pan2020decomposing,pan22decomposing} have proposed an approach to decompose a monolithic model into modules to enable reusability and replaceability of the decomposed modules. Similarly, a more modular architecture can be proposed for the NLP-based systems so that instead of reusing the entire model, developers can use the parts of it.
%Also, there are works in the NLP domain about pruning~\cite{ao2020darb}, compression techniques~\cite{bucilua2006model}, etc., and we believe that there is still the need for additional research on reducing the model size.
\subsection{How processing bugs in NLP are different from traditional DL bugs?}
%\textbf{Discuss what is processing bug and what it looks like in traditional DL}.
Compared to the DL, NLP-based software suffers from bugs related to the correct algorithm and parameters to retrain the model.
\finding{14.9\% of the bugs in reusing models are related to the
	processing bugs.}
For instance, previously, we discussed an issue
(Figure~\ref{fig:rq1process}), where the developers could not finetune
the model for the language translation task (Spanish to English). The
translation works perfectly if the sentence length is large.
However, when the sentences are short, it predicts in different languages other
than the languages specified while finetuning the model. While the model might have
the knowledge of the third language, that is unnecessary for
the developer's need. Without knowing the underlying architecture, fixing such bugs
are not always possible. In fact, the situation is akin to what has been proposed by \citeauthor{parnas1976design}~\cite{parnas1976design} regarding the program family. In that work, Parnas argued that software could be reused either as a complete
program (that produces output given input) or as smaller
components (intermediate stages that may or may not produce output given input).
While reusing the complete program, the traits of
the ancestors are passed to the descendent program without the knowledge. Some of these traits are important, but not all. In the
previous example, the same happened. While reusing, the
descendent software receives knowledge of another language other than English
and Spanish, which is not necessary for this context. Such bugs are not that common in traditional DL, as reusability is not as common as in NLP-based software.
For traditional DL models, such bugs only account for 6.3\% of the total bugs. While investigating, we found that such bugs in traditional DL are due to confusion while choosing the correct algorithm to train the model. However, for NLP, it is mostly the black-box nature of the reuse.
%Since, developer are not neccessarily update the underlying algorithm of the model, such bugs mostly occur while changing the NL-specific parameters that are exposed towards the clients.
%Apart from that, we found that processing bugs in \bart
%are primary due to updating the models (55.6\%) and setting the correct NL
%specific parameters (13.9\%).

\textbf{\textit{Implications.}} %% The start of the following paragraph reads
%unconnected. I recommend replacing the "This is akin to" with another
%expression and rewriting the paragraph. I feel that you are making a very
%important point here. And it's hard to follow it.
To avoid such scenarios,
Parnas~\cite{parnas1976design} has suggested that one needs to reuse the intermediate stages of the
software and reuse only the required
information. While the notion of the complete program vs. intermediate program
has not been identified yet, work by~\citeauthor{pan2020decomposing}~\cite{pan2020decomposing, pan22decomposing} has
identified how these black-box models can be seen as a composition of
smaller black-boxes. Understanding these smaller black-boxes might help
researchers capture the model's intermediate representation and reuse that
instead of the complete models.
%\subsection{Logic Bugs}
%\finding{Logic bugs are mostly seen in code using \bert and \xlm models.}
%
%
%\textbf{\textit{Implications.}}




==> nlp (Version 920)/rq2.tex <==
\section{Common Root Causes}
\label{sec:rq2}
\input{tablerq2.tex}
%In the previous section, we identified the common types of bugs observed during pre-trained NLP models reuse. However, the reasons that caused the bugs cannot be understood. 
	\begin{figure*}[]
% 	\vspace{32pt}
	\centering
	\includegraphics[width=1.0\linewidth]{revisedTaxonomy.pdf}
	\caption{Classification of root causes of bugs in NLP pre-trained models}
	\label{taxo}
% 	\vspace{14pt}
\end{figure*}
\input{root.tex}
\begin{figure*}[!htp]
	\begin{subfigure}{.5\textwidth}
		\centering
		\includegraphics[, trim={2cm 7cm 0cm 5cm},width=0.5\linewidth]{rootcause.pdf}
		\caption{Distribution of root causes in NLP (labels $<$7.8\% are
			hidden)}
		\label{fig:rootcause}
	\end{subfigure}%
	\begin{subfigure}{.5\textwidth}
		\centering
		\includegraphics[, trim={2cm 7cm 0cm 5cm},width=0.5\linewidth]{rootcauseDL.pdf}
		\caption{Distribution of root cause types in DL (labels $<$7.1\% are hidden)}
		\label{fig:rootcauseDLs}
	\end{subfigure}
	\caption{Comparison between the root causes of NLP and DL bugs~\cite{islam2019comprehensive} and their distributions}
	\centering
\end{figure*} 
We found that the root causes are significantly different and very specific to the NLP-based software.
In Figure~\ref{fig:rootcause}, we show the high-level distribution of the different root causes. We also show the distribution of root causes that are prevalent in traditional DL-based software in Figure~\ref{fig:rootcauseDLs} based on bugs reported by \cite{islam2019comprehensive}. Comparing both figures, we can observe that the types and the distributions of root causes are significantly different. For instance, DL models are more prone to bugs when API changes. However, since NLP models are pre-trained with a version of API, users do not tend to change the version, resulting in fewer bugs. Also, most bugs in the NLP system are updating the model by retraining, refining weights, etc., which are not common in DL-based software. This section focuses on the main root causes of bugs in NLP-based models, which are not present in the traditional DL. 
%We discuss each such prevalent cause and how they are different from traditional DL software (if similar cases were found in DL).
%\begin{figure}[!htp]
%	\centering
%	\includegraphics[, trim={2cm 7cm 0cm 5cm},width=0.6\linewidth]{rootcause.pdf}
%	\caption{Distribution of Root causes. Labels $<$7.1\% are hidden.}
%	\label{fig:rootcause}
%\end{figure}
%
%\begin{figure}[h]
%	\centering
%	\includegraphics[width=0.8\columnwidth]{root-cause-chart.pdf}
%	\caption{Distribution of Root Causes for the NLP Models}
%	\label{fig:rootcausechart}
%\end{figure}
\input{modelUpdate.tex}
\input{NLParam.tex}
%\input{execution.tex}


==> nlp (Version 920)/rq3.tex <==
\section{Frequent Impacts}
\label{sec:rq3}
In this RQ, we study the common effects of the bugs while reusing NLP models. We found that the categories denoted by the prior work~\cite{islam2019comprehensive} suffice to represent the bugs in NLP. However, the distributions are not the same. For example, incorrect functionality (DL: 9.18\%) and memory out of bound (DL: 0.82\%) errors are more prevalent in NLP (16.0
\% and 6.4\%) than traditional deep learning software. The percentages of bugs that abruptly halt the program (68.3\%) and cause bad performance (8.1\%) are less frequent in NLP. First, we discuss each type of impact and highlight the variabilities.
\begin{figure}
	\centering
	\includegraphics[width=.95\linewidth]{newImpact}
	\caption{Classification of impacts}
	\label{fig:impactTaxo}
\end{figure}
\input{impact.tex}
\begin{figure}[htp]
	\centering
	\includegraphics[, trim={2cm 8cm 0cm 6cm},width=0.6\linewidth]{impact.pdf}
	\caption{Distribution of impacts (labels $\le$0.7\% are
		hidden)
	}
	\label{fig:impact}
\end{figure}


%\begin{figure}
%	\centering
%	\includegraphics[width=0.7\linewidth]{impacts.pdf}
%	\caption{Distribution of impacts of the bugs in NLP models}
%	\label{fig:impactdist}
%\end{figure}

\finding{Reusing a pre-trained model helps to reduce performance related bugs.}
Compared to the traditional DL software, developers prefer to reuse the pre-trained model in the NLP domain. One of the prominent reasons is to reuse the knowledge from the huge corpus utilized to train these models. The culture of reusing instead of building every solution has helped to reduce the performance-related issues significantly (in DL: 13.8\%, in NLP: 8.1\%). 
%From Figure~\ref{fig:impactdist}, we can observe that the distribution is very similar for all the models except \ctrl and \gpt. Further investigation shows that developers prefer to reuse the models without significant changes for these models. The bugs found for changing the NL-specific parameters are extremely low (10.53\%) compared to the average distribution of this category (23.4\%). 
Out of all the root causes, updating the models (47.5\%) and changing the NL-specific parameters (31.25\%) are the most prevalent reasons for bad performance. 

% %\textbf{\textit{Implications.}} Model reuse in our ML domain is not as popular as in NLP. It might be helpful to use the key .
% \begin{figure}[!htp]
% 	\includegraphics[width=.9\linewidth]{oom.png}
% 	\caption{Example bug causing memory out of bound~\cite{oombug}}
% 	\label{fig:oom}
% \end{figure}
% \finding{Memory-related bugs are seen very often.}
% Due to the large size of the models, the memory issues are significantly more observed than the traditional deep learning software. 
% For instance, we found that a developer
% reported out of memory while retraining \bert model on a large dataset (Figure~\ref{fig:oom}). In most cases, developers reduce the size of the dataset, reduce the batch size, vocabulary size, etc., or prune the network to reduce the total number of parameters. However, often pruning and finetuning a network leads to the increase of the size. For example, in an issue~\cite{finetuning2}, we found that the size of the model has increased $\sim$54\% after finetuning. The solution
% to the issue has suggested that not all finetuning or pruning leads
% to the reduction of size; some use of parameters, e.g., Adam as an
% optimizer, increases the size of the model significantly. Moreover, the memory-out-of-bound bugs are mostly caused by the wrong choice of algorithm (21.88\%) or NL-specific parameters (51.86\%). 
% %\begin{figure}[!htp]
% %	\includegraphics[width=.9\linewidth]{finetuning2.png}
% %	\caption{Finetuning often leads to negative effects.~\cite{finetuning2}}
% %	\label{fig:finetuning2}
% %\end{figure}

% \textbf{\textit{Implications.}}
% In general, neural network based software are data or computation intensive and hence require powerful computational platforms. Since NLP pre-trained models are memory intensive, task parallelization and concurrent programming paradigm would be required. Furthermore, the libraries should mention memory requirements in their APIs. Finally, more dynamic analyses are required to catch memory bugs in the earlier stage of development. 



==> nlp (Version 920)/rq4.tex <==
%\section{Correlation among Bugs}
%\label{sec:rq4}

==> nlp (Version 920)/tablerq2.tex <==
%% Table generated by Excel2LaTeX from sheet 'Sheet16'
%\begin{table*}[htbp]
% 	\centering
% \vspace{25pt}
% \caption{Distribution of Root Cause and Impacts.}
% \setlength{\tabcolsep}{3pt}
% \rowcolors{2}{gray!25}{white}
%    \begin{tabular}{|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|}
%    	\hline
%    	\rowcolor{gray!50} \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model Name}}} & \multicolumn{8}{c}{Root Cause}     & \multicolumn{6}{c}{Impacts} \\
%    	\rowcolor{gray!50}  &\multicolumn{1}{l}{\textbf{MR}} & \multicolumn{1}{l}{\textbf{CLSP}} & \multicolumn{1}{l}{\textbf{EE}} & \multicolumn{1}{l}{\textbf{APIM}} & \multicolumn{1}{l}{\textbf{Arch}} & \multicolumn{1}{l}{\textbf{DF}} & \multicolumn{1}{l}{\textbf{Alg}} & \multicolumn{1}{l}{\textbf{PE}} & \multicolumn{1}{l}{\textbf{Crash}} & \multicolumn{1}{l}{\textbf{IF}} & \multicolumn{1}{l}{\textbf{BP}} & \multicolumn{1}{l}{\textbf{OOM}} & \multicolumn{1}{l}{\textbf{Hang}} & \multicolumn{1}{l}{\textbf{DC}} \\
%    \hline
%    \hline
%    ALBERT & 33.3\% & 21.6\% & 11.8\% & 15.7\% & 7.8\% & 3.9\% & 3.9\% & 2.0\% & 84.3\% & 5.9\% & 9.8\% & 0.0\% & 0.0\% & 0.0\% \\
%    \hline
%	Bart  & 47.0\% & 20.0\% & 5.0\% & 9.0\% & 12.0\% & 2.0\% & 2.0\% & 3.0\% & 63.0\% & 19.0\% & 8.0\% & 10.0\% & 0.0\% & 0.0\% \\
%	\hline
%	Bert  & 29.5\% & 33.8\% & 9.7\% & 9.2\% & 4.8\% & 10.6\% & 0.5\% & 1.9\% & 65.7\% & 16.4\% & 10.1\% & 6.8\% & 0.5\% & 0.5\% \\
%	\hline
%	CTRL  & 8.0\% & 28.0\% & 20.0\% & 24.0\% & 4.0\% & 12.0\% & 4.0\% & 0.0\% & 72.0\% & 12.0\% & 0.0\% & 16.0\% & 0.0\% & 0.0\% \\
%	\hline
%	GPT-2 & 24.3\% & 4.3\% & 31.4\% & 18.6\% & 7.1\% & 7.1\% & 5.7\% & 1.4\% & 77.1\% & 18.6\% & 0.0\% & 4.3\% & 0.0\% & 0.0\% \\
%	\hline
%	RoBERTa & 39.9\% & 12.3\% & 14.5\% & 6.5\% & 14.5\% & 2.9\% & 6.5\% & 2.9\% & 62.3\% & 25.4\% & 7.2\% & 2.9\% & 0.7\% & 1.4\% \\
%	\hline
%	T5    & 40.5\% & 11.1\% & 19.0\% & 6.3\% & 10.3\% & 5.6\% & 2.4\% & 4.8\% & 68.3\% & 15.1\% & 12.7\% & 1.6\% & 2.4\% & 0.0\% \\
%	\hline
%	Transformer-XL & 22.2\% & 27.8\% & 11.1\% & 16.7\% & 0.0\% & 22.2\% & 0.0\% & 0.0\% & 50.0\% & 0.0\% & 22.2\% & 27.8\% & 0.0\% & 0.0\% \\
%	\hline
%	XLM   & 19.3\% & 50.6\% & 12.0\% & 2.4\% & 7.2\% & 7.2\% & 1.2\% & 0.0\% & 54.2\% & 18.1\% & 14.5\% & 12.0\% & 1.2\% & 0.0\% \\
%	\hline
%	XLNET & 19.1\% & 27.7\% & 17.0\% & 4.3\% & 4.3\% & 27.7\% & 0.0\% & 0.0\% & 76.6\% & 10.6\% & 0.0\% & 12.8\% & 0.0\% & 0.0\% \\
%    \hline
%    \hline
%   \textbf{Total} & \textbf{32.3\%} & \textbf{23.4\%} & \textbf{14.1\%} & \textbf{9.1\%} & \textbf{8.4\%} & \textbf{7.9\%} & \textbf{2.7\%} & \textbf{2.2\%} & \textbf{66.6\%} & \textbf{16.9\%} & \textbf{8.8\%} & \textbf{6.7\%} & \textbf{0.7\%} & \textbf{0.3\%} \\
%\hline   \end{tabular}%
%  \label{tb:root}%
%\end{table*}%

==> nlp (Version 920)/threat.tex <==
\section{Threats To Validity}
\label{sec:threat}

%% you need to explain why the threat is a threat and how you mitigate it. Otherwise, it sounds like you either don't understand the threat or you don't care.
%% both have severe consequences for the work and its validity.
%% Only two threats? One internal and another external?
\textbf{Internal Threat.} 
The finding and the implications are drawn based on the classification scheme developed. To remove the threat regarding the quality of the classification scheme, we adapted the base scheme from prior works and added categories based on an open coding approach. The classification scheme was developed by two researchers and with rigorous discussions, which is the same way prior works~\cite{islam2019comprehensive, islam2020repairing, zhang2018empirical} have developed their classification schemes. Also, to remove the researcher's bias, we compute the Cohen's Kappa coefficient to measure the agreement. Only when the perfect agreement was achieved, the raters labeled the post individually. Moreover, any discrepancies were resolved over a discussion.

%One threat to this study can be the classification scheme, researchers bias, and confirmation bias. For the classification scheme, especially for bug type and impacts, we adapted the scheme from prior works. 
%% why the above is a threat? how did you mitigate the threat?
%For root cause, two raters individually did a pilot study and applied an open coding scheme to fix the labels. 
%%% this should be the past. The study is over
%To mitiage the other two threats, raters discussed among themselves to clear any confusion. Furthermore, we computed Cohen's Kappa coefficient to measure the agreement. Only when the perfect agreement was achieved, the raters labeled the post individually. Moreover, any discrepancies were resolved over a discussion.

\noindent\textbf{External Threat.}
%% you **mitigate** a threat. Why is this a threat?
The quality of the issues mined can be an external threat. To mitigate, we selected the most popular NLP models from a vastly used framework (Huggingface Transformer). Then, instead of selecting the issues that are related to bugs in \textit{Huggingface Transformer}, we mine the bugs found while using these NLP models. Then, we removed \gh repositories that are not well-maintained (number of issues $\le$50) and selected the popular ones (based on star count). We mined the bug-related issues using keywords proposed by the prior work~\cite{garcia2020comprehensive} and labeling done by the maintainer of the repositories. After mining such issues, raters validated whether the issue was related to a bug or not by manual verification. %% Add the reference for prior work

==> nlp (Version 920)/to-do.tex <==
%1. Introduction more discussion on comparsion with prior work.
%2. Pictorial representation of islam etal vs our work. -- Rangeet
%3. Definition table. -- Sumon
%4. Include definition in the RQ -- Rangeet
%5. Break the RQs for relevant findings. -- Rangeet and Sumon
%6. NLP study in 2021 -- Add reference (TOSEM reference) -- Breno
%7. Add new models (try) -- Breno
%8. Cover letter
%9. Finding distribution to check the validity of the claim. -- All
%
%Comments:
%1. No data to support the claim.
%2. Make the claim actionable
%3. Incremental (Islam et al, Zhang et al., Gunel et al.)


==> nltable.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet18'
\begin{table}[htbp]
\centering
\vspace{5pt}
\caption{Distribution of Language Specific Parameters}
\setlength{\tabcolsep}{3pt}
\rowcolors{2}{gray!25}{white}
    \begin{tabular}{|l|r|r|r|r|r|r|r|}
    	\hline
    		\rowcolor{gray!50}
     \textbf{Model} & \textbf{Batch} & \textbf{Token} & \textbf{Lang} & \textbf{ML} & \textbf{Vocab} & \textbf{Sen} & \textbf{Others} \\
    \hline
    \hline
    ALBERT & 9.1\% & 36.4\% & 0.0\% & 9.1\% & 27.3\% & 0.0\% & 18.2\% \\
    \hline
    Bart  & 10.0\% & 25.0\% & 35.0\% & 20.0\% & 0.0\% & 5.0\% & 5.0\% \\
    \hline
    Bert  & 25.7\% & 24.3\% & 14.3\% & 18.6\% & 14.3\% & 2.9\% & 0.0\% \\
    \hline
    CTRL  & 42.9\% & 14.3\% & 0.0\% & 0.0\% & 42.9\% & 0.0\% & 0.0\% \\
    \hline
    GPT-2 & 0.0\% & 0.0\% & 0.0\% & 66.7\% & 33.3\% & 0.0\% & 0.0\% \\
    \hline
    RoBERTa & 0.0\% & 35.3\% & 23.5\% & 5.9\% & 5.9\% & 29.4\% & 0.0\% \\
    \hline
    T5    & 21.4\% & 35.7\% & 14.3\% & 21.4\% & 7.1\% & 0.0\% & 0.0\% \\
    \hline
    T-XL & 20.0\% & 0.0\% & 0.0\% & 40.0\% & 40.0\% & 0.0\% & 0.0\% \\
    \hline
    XLM   & 28.6\% & 7.1\% & 23.8\% & 11.9\% & 26.2\% & 2.4\% & 0.0\% \\
    \hline
    XLNET & 46.2\% & 23.1\% & 15.4\% & 15.4\% & 0.0\% & 0.0\% & 0.0\% \\
    \hline
    \hline
    \textbf{Total} & \textbf{22.8\%} & \textbf{21.8\%} & \textbf{17.3\%} & \textbf{16.3\%} & \textbf{15.8\%} & \textbf{4.5\%} & \textbf{1.5\%} \\
    \hline
    \end{tabular}%
  \label{tb:language}%
\end{table}%



==> overview.tex <==
\section{Natural Language Processing Systems}
\label{sec:nlp}
\begin{figure*}
	\includegraphics[, width=1\linewidth]{overview.pdf}
	\caption{The Workflow of Reusing Pre-Trained Models for Natural Language
		Processing Tasks.}
	\label{fig:overview}
\end{figure*}
Before we begin the bug-related discussion, we briefly discuss common components involving reusing a pre-trained model. Figure \ref{fig:overview} shows the traditional workflow, which is what most developers follow for reusing models. Broadly, the components are classified into, 1) data
preprocessing, 2) reusing models, and 3) task customization.


\textbf{Data Preprocessing.} 
The data preprocessing can be done on the training data of the pre-trained models or the domain-specific dataset. Since the training dataset is not readily available to the developer while reusing, we consider it as a black box component (grey boxes in Figure \ref{fig:overview}). At this stage, an initial transformation of the free-form text is
performed. The transformation includes tokenization, normalization, removal of %% I feel that the transformation should have all the steps listed here
unwanted segments, etc. These transformations will help attain a better feature representation of the raw data that can be used later. %These transformations 
%will help the raw data for better feature representation

\textbf{Reusing Pre-trained Model.}
At this stage, the pre-trained models are reused in any of the three ways:
\begin{itemize}[leftmargin=*]
	\item Without any change: These models can be reused without any alteration to the input or output. For instance, the GitHub issue discusses how the \bert model can directly be reused.
	\item Transfer learning: In this setting, the model pre-trained on one task is used for a different task. It helps in adding new abilities to the model without having to re-train from scratch.
	\item Fine-tuning: In this setting, the models are re-trained on the domain-specific dataset to capture the task-specific features. In comparison to transfer learning, here, only hyper-parameters are optimized for a specific pre-trained model.
\end{itemize}
%% Consider rewriting the following paragraph and including additional explanation about "the needs"
%% if you start a list with "e.g.," there's no need to put "etc." at the end.
\textbf{Task Customization.} In this stage, downstream tasks, e.g., sentiment 
analysis, opinion mining, information retrieval~(\cite{tang2016aspect,
	rush2015neural}). Broadly, we can categorize the modeling technique either as a single-task or
multi-task model. Single-task models address applications (Task 1, Task 2,
\dots, Task $n$) as independent components, whereas multi-task models address
multi-applications by leveraging synchronization through interfaces between
them. 

==> parameter.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet12'
\begin{table}[htbp]
%\begin{wraptable}{R}{0.5\linewidth}
	\centering
  \small
	%\vspace{25pt}
	\caption{Pre-trained Models' Description.}
	\setlength{\tabcolsep}{3pt}
	\rowcolors{2}{gray!25}{white}
    \begin{tabular}{|c|c|c|c|}
    \hline
    \rowcolor{gray!50} \textbf{Year} & \textbf{Model} & \textbf{Parameters} \\
    \hline
    \hline
    2019 & \albert & 223M \\
    \hline
    2019 & \bart  & 406M\\
    \hline
    2018 & \bert  & 340M\\
    \hline
    2019 & \ctrl  & 1.6B\\
    \hline
    2019 & \gpt & 1.5B\\
    \hline
    2019 & \roberta & 355M\\
    \hline
    2019 & \tf    & 11B\\
    \hline
    2019 & \txl & 257M\\
    \hline
    2019 & \xlm   & 500M\\
    \hline
    2019 & \xlnet & 340M\\
    \hline
    \end{tabular}%
  \label{tb:modelsize}%
\end{table}%
%\end{wraptable}


==> reusetable.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet19'
\begin{table}[thbp]
	\centering
  \footnotesize
	\vspace{5pt}
	\caption{Distribution of Bugs due to Updating the Pre-trained Models}
	\setlength{\tabcolsep}{3pt}
	\rowcolors{2}{gray!25}{white}
    \begin{tabular}{|l|r|r|r|r|r|r|}
    		\rowcolor{gray!50}
    		\hline
    \textbf{Model} & \multicolumn{1}{c|}{\textbf{Migration}} & \multicolumn{1}{c|}{\textbf{Retrain}} & \multicolumn{1}{c|}{\textbf{Fine Tuning}} & \multicolumn{1}{c|}{\textbf{Checkpoint}} & \multicolumn{1}{c|}{\textbf{Refine Weight}} \\
    \hline
    \hline
    ALBERT & 23.53\% & 47.06\% & 17.65\% & 11.76\% & 0.00\%\\
    \hline
    Bart  & 19.15\% & 29.79\% & 31.91\% & 19.15\% & 0.00\%\\
    \hline
    Bert  & 39.34\% & 18.03\% & 11.48\% & 31.15\% & 0.00\%\\
    \hline
    CTRL  & 50.00\% & 0.00\% & 50.00\% & 0.00\% & 0.00\%\\
    \hline
    GPT-2 & 88.24\% & 0.00\% & 0.00\% & 11.76\% & 0.00\%\\
    \hline
    RoBERTa & 30.91\% & 41.82\% & 18.18\% & 7.27\% & 1.82\%\\
    \hline
    T5    & 13.73\% & 43.14\% & 27.45\% & 15.69\% & 0.00\%\\
    \hline
    T-XL & 50.00\% & 50.00\% & 0.00\% & 0.00\% & 0.00\% \\
    \hline
    XLM   & 62.50\% & 12.50\% & 12.50\% & 6.25\% & 6.25\% \\
    \hline
    XLNET & 44.44\% & 22.22\% & 22.22\% & 11.11\% & 0.00\% \\
    \hline
    \hline \textbf{Total} & \textbf{33.33\%} & \textbf{30.11\%} & \textbf{19.35\%} & \textbf{16.49\%} & \textbf{0.72\%} \\
    \hline
    \end{tabular}%
  \label{tb:reuse}%
\end{table}%


==> rq4.tex <==
%\section{Correlation among Bugs}
%\label{sec:rq4}
